PAC Mode Estimation using PPR Martingale Confidence Sequences

We consider the problem of correctly identifying the \textit{mode} of a discrete distribution $\mathcal{P}$ with sufficiently high probability by observing a sequence of i.i.d. samples drawn from $\mathcal{P}$. This problem reduces to the estimation of a single parameter when $\mathcal{P}$ has a support set of size $K = 2$. After noting that this special case is tackled very well by prior-posterior-ratio (PPR) martingale confidence sequences \citep{waudby-ramdas-ppr}, we propose a generalisation to mode estimation, in which $\mathcal{P}$ may take $K \geq 2$ values. To begin, we show that the "one-versus-one" principle to generalise from $K = 2$ to $K \geq 2$ classes is more efficient than the "one-versus-rest" alternative. We then prove that our resulting stopping rule, denoted PPR-1v1, is asymptotically optimal (as the mistake probability is taken to $0$). PPR-1v1 is parameter-free and computationally light, and incurs significantly fewer samples than competitors even in the non-asymptotic regime. We demonstrate its gains in two practical applications of sampling: election forecasting and verification of smart contracts in blockchains.

==> NeurIPS submission/abstract.tex <==
\begin{abstract}
We consider the problem of correctly identifying the \textit{mode} of a discrete distribution $\mathcal{P}$ with sufficiently high probability by observing a sequence of i.i.d. samples drawn according to $\mathcal{P}$. This problem reduces to the estimation of a single parameter when $\mathcal{P}$ has a support set of size $K = 2$. Noting the efficiency of prior-posterior-ratio (PPR) martingale confidence sequences \cite{waudby-ramdas-ppr} for handling this special case, we propose a generalisation to mode estimation, in which $\mathcal{P}$ may take $K \geq 2$ values. We observe that the ``one-versus-one'' principle yields a more efficient generalisation than the ``one-versus-rest'' alternative. Our resulting stopping rule, denoted PPR-ME, is optimal in its sample complexity up to a logarithmic factor. Moreover, PPR-ME empirically outperforms several other competing approaches for mode estimation. We demonstrate the  gains offered by PPR-ME in two practical applications: (1) sample-based forecasting of the winner in indirect election systems, and (2) efficient verification of smart contracts in permissionless blockchains. 

\end{abstract}

==> NeurIPS submission/packages.tex <==
% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2021

% ready for submission
% \usepackage{neurips_2021}
% \PassOptionsToPackage{numbers}{natbib}
% \usepackage[preprint]{neurips_2021}

% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
    % \usepackage[preprint]{neurips_2021}

% to compile a camera-ready version, add the [final] option, e.g.:
    % \usepackage[final]{neurips_2021}

% to avoid loading the natbib package, add option nonatbib:
    \usepackage[preprint,nonatbib]{neurips_2021}
% \usepackage[numbers]{natbib}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{float}
\usepackage{epstopdf}
\usepackage{esvect}
\usepackage{amsmath}
\usepackage{algorithm2e}
\usepackage{siunitx}
\usepackage{caption, subcaption}
\usepackage{geometry}
\usepackage{amsfonts} 
\usepackage{dsfont}
\usepackage{mathtools}
% \usepackage[ruled,vlined]{algorithm2e}
% \usepackage{algorithmic}
\usepackage{rotating}
\usepackage[noend]{algpseudocode}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{graphicx}
\usepackage{dsfont}
% \usepackage{algorithm}
% \usepackage[noend]{algorithmic}
\usepackage{caption,subcaption}
\usepackage{mathtools}
\usepackage{marginnote}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}


==> NeurIPS submission/sections/blockchains.tex <==
\section{Application: Verifying Smart Contracts in Permissionless Blockchains}
\label{sec:blockhains}

Our second application of PAC mode estimation is in a domain of growing contemporary relevance. Permissionless blockchains such as Bitcoin~\cite{NakamotoBitcoin} and Ethereum~\cite{buterin2014} %\vinay{Bitcoin does not easily allow smart contracts. Ethereum does allow them.}
allow uncertified agents to join a pool of service providers, also called \textit{nodes}.
%\vinay{In the YODA setup, there are the usual miners who normally execute all smart contracts of Ethereum. If there were no computationally intensive smart contracts then we would not need any other nodes. Ethereum does not support computationally intensive smart contracts at this time. In YODA we proposed an additional set of volunteer nodes to execute these computationally intensive smart contracts. I am not sure if we should distinguish between miners and these other volunteer nodes in this paper though.}
A recent feature that has emerged in such blockchains is the execution of ``smart contracts''~\cite{sourav2019,buterin2014}, which could include, for example, running computationally-heavy jobs such as machine learning algorithms. In an ideal world, a client who requires a computation to be performed can simply enter into a smart contract with some particular node in the blockchain, and pay a transaction cost for the service. Unfortunately, there is no guarantee that nodes in a permissionless blockchain are honest. A ``Byzantine''
%\sd{Is the term "byzantine" common in AI community? If not, we can change this to "malicious".}
(or \textit{malicious}) node could easily return a quick-to-compute, incorrect output, to the detriment of the client. 

In recent work, Das et al.~\cite{sourav2019} propose an approach for the \textit{probabilistic verification} of smart contracts. Abstractly, assume that the computation to be performed for the client is deterministic, and it has a (yet unknown) output $o_{\text{correct}}$. The proposed model accommodates any blockchain in which the fraction of Byzantine nodes is at most $f_{\max} \in [0, \frac{1}{2})$. With this assumption, it becomes feasible to give a probabilistic guarantee on obtaining the correct output. For any fixed mistake probability $\delta \in (0, 1)$, the client could ship out the computation to  $\Theta\left(\frac{1}{(\frac{1}{2} - f_{\max})^{2}}\log(\frac{1}{\delta})\right)$
%\vinay{I don't recalling having this $\Theta$ result in YODA}
nodes, and take their majority response as the answer, thereby ensuring $\delta$-correctness. Unfortunately, transaction costs can be substantial, especially those for computationally-intensive contracts. Hence, it is in the client's interest to minimise the number of nodes queried to achieve the same probabilistic guarantee. For example, a sequential procedure could potentially query fewer nodes if $f \ll f_{\max}$.

\subsection{Comparison with SPRT}
\label{subsec:comparisonwithsprt}


Our contribution in the context of this application is to propose PPR-ME as an alternative to Wald's Sequential Probability Ratio Test (SPRT)~\cite{awald1945}, which is used by Das et al.~\cite{sourav2019} for their verification procedure. This classical test finds use in many other engineering applications~\cite{kenny1991,chen2008}, some of which could also benefit from the advantages of PPR-ME over SPRT.

To apply SPRT for verifying smart contracts, Das et al.~\cite{sourav2019} assume that out of the total of $N$ nodes in the blockchain, batches of size $m$, chosen uniformly at random, can be queried in sequence.
%\sd{The term "step" is introduced suddenly. May be start with "The approach of [22] proceeds in steps, where a subset of nodes are sampled in each step"?}.
For simplicity assume the answers returned are from the set $\{0, 1, 2, \dots\}$. Let $q = \frac{m}{N}$, and $c_{i,t}$ be the number of times answer $i$ is reported in the $t^{th}$ step, $i \geq 0$, $t \geq 1$. Defining $l_{i,T} = \sum_{t=1}^{T} (2c_{i,t} - m)m$, a derivation~\cite{sourav2019} establishes that $\delta$-correct SPRT stops at time $T$, giving $i$ as the answer if
\begin{equation*}
    l_{i,T} > \ln\left ( \frac{1 - \delta}{\delta} \right) \frac{2q(1-q)N (1 - f_{\max})f_{\max}}{1 - 2f_{\max}}.
\end{equation*}
The primary disadvantage of SPRT in this context is the need for the user to provide $f_{\max}$, which is used in the stopping rule.
%\sj{Isn't the need of a large $m$ to be $\delta$-correct also a disadvantage? Whereas we give provable $\delta$-correctness with similar sample complexity}
While a lower value of $f_{\max}$ will improve the efficiency of the rule, unfortunately $\delta$-correctness no longer holds if $f$, the true fraction of Byzantine nodes, exceeds $f_{max}$. Figure~\ref{fig:fmax-underestimate} plots the empirical error made by SPRT (averaged over 50,000 runs) on a problem instance in which the Byzantine nodes all give the same (incorrect) answer. We fix $f_{\max} = 0.1$, and plot the error for different settings of $f$. The blockchain has $N = 1600$ nodes, of which SPRT samples $m = 20$ at a time. Although the test is run using  mistake probability $\delta = 0.005$, observe that the empirical error exceeds $\delta$ when $f > f_{\max}$.
%\vinay{I don't see any error bars in the Figure? Would that hurt?}

Since the verification task at hand is precisely that of PAC mode estimation, PPR-ME becomes a viable alternative, especially since it does not need the knowledge of $f_{\max}$. In fact, PPR-ME can identify the mode even if its associated probability is less than $\frac{1}{2}$ (although in this case, it can no longer be guaranteed that the mode is $o_{\text{correct}}$, since the Byzantine nodes may collude). Observe from Figure~\ref{fig:fmax-underestimate} that unlike SPRT, the empirical error rate of PPR-ME (equivalent to PPR-Bernoulli since we have set $K = 2$) remains within $\delta$ even for $f > f_{\max}$.

In Figure~\ref{fig:adaptiveK}, we compare the sample complexities of PPR-ME and SPRT. Whereas other problem parameters (including $f_{max}$) stay the same as before, we consider an instance in which $K = 10$.
%\vinay{I seem to have missed what "K" is. Haven't read the first 4 sections. I assume it is from there.}
The single correct answer is given by a $(1 - f)$-fraction of the nodes, while $9$ different incorrect answers are given by the Byzantine nodes, each equally common. The version of SPRT used is a 1vr
%\vinay{What is 1vr?}
adaptation of the basic procedure~\cite{sourav2019} to $K = 10$. First, we observe that SPRT terminates before PPR-1v1 and PPR-1vr at all values of $f$. The PPR algorithms pay this price for having to assure $\delta$-correctness at all values of $f < \frac{1}{2}$, unlike SPRT, which does so only for $f < f_{max}$. We show the performance of another PPR variant, denoted ``PPR-Adaptive'', in the same plot. In reality, we cannot be sure about the number of answers $K$ that will be returned by the blockchain's nodes--and hence cannot use it in our stopping rule. Under PPR-Adaptive, which is a 1v1 strategy, the overall mistake probability $\delta$ is divided into the \textit{infinite} sequence $k \frac{\delta}{1^{2}}, k \frac{\delta}{2^{2}}, k \frac{\delta}{3^{2}}, \dots$ (with $k = \frac{6}{\pi^{2}}$). Whenever a new answer is revealed, it is inserted into the list of possible answers, and its pairwise tests given mistake probabilities from the unused portion of the sequence. In principle, PPR-Adaptive can accommodate any number of answers, incurring only a small increase in sample complexity, as visible from Figure~\ref{fig:adaptiveK}.



%In this section, we present an application of mode estimation in a completely different domain of verifying smart contracts in permission less blockchains. The problem can be stated as follows - we want to evaluate a deterministic function $\boldsymbol{\Psi}$ and there are a total of $N$ nodes which can be queried to evaluate the function. The nodes can be divided into two types - \emph{honest} nodes which evaluate the function correctly when queried and \emph{byzantine} nodes which can be thought of as adversaries and return a wrong evaluation of the function. The goal is to correctly evaluate the function while minimizing the number of queries to be made. It is assumed that the maximum fraction of byzantine nodes $f_{max}$ is $< 1/2$ which gives us the hope to find the correct answer. The true fraction of byzantine nodes $f \leq f_{max}$ is however unknown.\newline

%We compare our approach with the SPRT stopping rule which is shown to be optimal for the above problem [CITE]. Let $m$ be the number of set of nodes queried at each time step which is known as the execution set. SPRT considers the ratio of the likelihood of two hypotheses (answer to be correct or incorrect) and stops when this exceeds $(1 - \delta)/\delta$. More formally, let $q = m/N$ and $c_{i,k}$ be the number of times answer $c_i$ was reported in the $k^{th}$ iteration. Defining $l_{i,T} = \sum_{t=1}^{T} (2c_{i,t} - m)m$, SPRT stops at time $T$ giving $c_i$ as the answer which is correct with probability at least $1 - \delta$ if
\begin{comment}
\begin{equation*}
    l_{i,T} > \text{log}\left ( \frac{1 - \delta}{\delta} \right) \frac{2q(1-q)N (1 - f_{max})f_{max}}{1 - 2f_{max}}
\end{equation*}
The issue with SPRT is that one needs to knowledge of $f_{max}$ and the correctness relies on the fact that the true fraction of the byzantine nodes $f$ is smaller than $f_{max}$. On the other hand, PPR does not need any such information and guarantees $\delta$ correctness in all regimes.
\end{comment}

\begin{figure}[t]
    \centering
    \subfloat[\centering $K  = 2$ (single adversarial answer)]{{\includegraphics[width=6.7cm]{figures/error_bchn.png} 
    }
    \label{fig:fmax-underestimate}
    }%
    % \qquad
    \subfloat[\centering $K = 10$  ]{{\includegraphics[width=6.7cm]{figures/samples_byz_final.png}
    }
    \label{fig:adaptiveK}
    }%

    \caption{Comparisons with SPRT for the probabilistic verification of smart contracts, obtained with parameter settings
    $N = 1600$, $m = 20$, $\delta = 0.005$, $f_{max} = 0.1$. Plot (a) shows the empirical error rates of the algorithms as the true Byzantine fraction $f$ is varied, taking $K = 2$. Plot (b) shows the sample complexity of various algorithms against varying $f$, on an instance with $K = 10$ answers.}%
    \label{fig:blockchain}%
\end{figure}
%In our experiments, we set $N = 1600$ and $f_{max} = 0.1$. We assume that all the adversaries give the same incorrect evaluation of the function which would make the problem hardest. We vary $f$ from $0.05$ to $0.4$ mainly with the aim to study under specification of $f_{max}$ for the problem at hand. The above plots are averaged over $50,000$ runs. Figure~\ref{fig:blockchain}a suggests that as $f$ increases, SPRT error also increases overshooting the $\delta = 0.05$ limit while PPR is still correct for all values of $f$. Regarding the sample complexities as shown in Figure~\ref{fig:blockchain}b, we see that PPR is not that far from SPRT given that is has no additional knowledge and always outputs the correct value of the function which is important due to security reasons in the mentioned application.\newline
% \begin{figure}[H]
%     \centering
%     \includegraphics[width = 7cm]{figures/multi_answer.png}

%     \caption{$m = 20$, $\delta = 0.005$, $f_{max} = 0.1$ }%
%     \label{fig:block2}
% \end{figure}
%Next, we study the case when the byzantine nodes can give an evaluation of the function from upto $9$ incorrect answers. Thus, this can be thought of as the case of $K = 10$ using our notation. SPRT needs knowledge of this $K$ which can be handled by our framework named PPR-Adaptive. In this, on seeing the $kth$ new answer, we assign it's confidence sequence an error probability of $6\delta/(k\pi)^2$ which ensures that union bound over all $k$ is still less than $\delta$. PPR-ME and PPR-EVR are implemented assuming the knowledge of $K$ as discussed in the previous sections. 
%\jv{For multi answer case, none of the algorithms make any error so need to think whether the plot is meaningful. The adaptively allocating error budgets can be put even in the main text while describing PPR}

% \jv{The issue is correctness of SPRT assumes the execution set is large and in practice it does violate the $\delta = 0.01$ error bound. But large execution set simply means the same number of nodes samples by all algorithms in the low $f$ regime}
% Some instances where SPRT makes errors for $f> f_{max}$(averaged over 1000 runs): [see plots for $f < f_{max}$]
% \begin{enumerate}
%     \item $f_{max} = 0.1, f = 0.2, \delta = 0.01, m = 10$: SPRT accuracy 0.986000 samples 6.780000
%     \item $f_{max} = 0.1, f = 0.2, \delta = 0.01, m = 10$: PPR accuracy 1.000000 samples 9.165000
%     \item $f_{max} = 0.1, f = 0.3, \delta = 0.01, m = 20$: SPRT accuracy 0.980000 samples 12.118000
%     \item $f_{max} = 0.1, f = 0.3, \delta = 0.01, m = 20$: PPR accuracy 0.996000 samples 16.842000
    
% \end{enumerate}
% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.25]{figures/plot_1_m1.png}
%     \caption{Comparison of various algorithms for blockchain application for $\delta = 0.01$}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.25]{figures/plot_smalldelta.png}
%     \caption{Comparison of various algorithms for blockchain application for $\delta = 10^{-8}$}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \subfloat[\centering Accuracy averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_error_m.png} }}%
%     % \qquad
%     \subfloat[\centering Samples averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_samples_m.png} }}%
%     \caption{m = 2, $\delta = 0.01$, $f_{max} = 0.45$ }%
%     \label{fig:m1}%
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \subfloat[\centering Accuracy averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_error_m5.png} }}%
%     % \qquad
%     \subfloat[\centering Samples averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_samples_m5.png} }}%
%     \caption{m = 5, $\delta = 0.01$, $f_{max} = 0.45$ }%
%     \label{fig:m1}%
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \subfloat[\centering Accuracy averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_error_m5_1e-4.png} }}%
%     % \qquad
%     \subfloat[\centering Samples averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_samples_m5_1e-4.png} }}%
%     \caption{m = 5, $\delta = 10^{-4}$, $f_{max} = 0.45$ }%
%     \label{fig:m1}%
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \subfloat[\centering Accuracy averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_error_m20.png} }}%
%     % \qquad
%     \subfloat[\centering Samples averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_samples_m20.png} }}%
%     \caption{m = 20, $\delta = 0.01$, $f_{max} = 0.45$ }%
%     \label{fig:m1}%
% \end{figure}


==> NeurIPS submission/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we apply the framework of PPR martingale confidence sequences to the problem of PAC mode estimation. Our investigation follows two different dimensions that play a significant role in determining the efficiency of stopping rules. First is the tightness of the confidence bounds used internally in the stopping rule. By separately focusing on the Bernoulli case, we show that the PPR martingale stopping rule is sample-efficient both in theory and in practice. Our analysis as well as experiments may be of independent interest to research on pure exploration problems in stochastic bandits. The second aspect of mode estimation is the template applied to generalise from $K = 2$ to $K \geq 2$, which can typically be applied with any valid confidence bounds. Of the two major choices---``one-versus-one'' (1v1) and ``one-versus-rest'' (1vr)---we find 1v1 to be the more efficient. 

The PPR-ME algorithm that combines both ideas is simple, computationally efficient, yet significantly more sample-efficient not only than the recently-proposed $\mathcal{A}_{1}$ algorithm~\cite{Shah_Choudhury_Karamchandani_Gopalan_2020}, but many other baselines (including an improved variant of $\mathcal{A}_{1}$ that we include in our experiments). To illustrate the practical relevance of PPR-ME, we present two separate real-world applications in which it can offer significant advantages over earlier approaches. In sample-based election forecasting, PPR-ME significantly reduces the sample complexity when paired with the DCB sampling strategy. Analysing the sample complexity of DCB in terms of its problem parameters remains an avenue for future work, which could contribute to a growing literature on sample-based techniques in social choice theory~\cite{dey2015,pmlr-v37-rajkumar15}. Our second application, to probabilistic verification in blockchains, is based on PPR-ME being relatively assumption-free, which makes it a promising algorithm for many industrial applications.

\begin{comment}
technical prior known to be hard  analysus of dcb, even moe efficient with modeling structure other industrial applications.

add bib of lihong li's prior analysis paper. \dm{added cite as \cite{che2016}}

Generalized Likelihood Ratio Test (\textbf{GLR}) \cite{pmlr-v49-garivier16a}: This work defines the Chernoff stopping rule which involves computing the GLR statistic $Z_{a, b}(t)$ for all arms/parties $a$ and $b$. $Z_{a, b}(t)$ can be thought of as the log of the likelihood ratios of two hyoptheses and the stopping rule when the max over $a$ and $b$ of $Z_{a, b}(t)$ is more than some threshold.

\end{comment}


==> NeurIPS submission/sections/elections.tex <==
\section{Application: Winner-forecasting in Indirect Elections}
\label{sec:elections}

Opinion polls---deployed  to gauge public perception of competing products in a market, or to forecast the winner of an upcoming election---are a natural application of mode estimation. In fact, the algorithms discussed in Section~\ref{sec:ppr-me} can all be applied with only minor alterations to  \textit{plurality} systems, wherein the task is precisely that of determining the choice preferred by the largest fraction of the target population. Waudby-Smith and Ramdas~\cite{waudby-ramdas-ppr} illustrate the use of PPR martingale confidence sequences precisely on this application. Specifically they consider the construction of confidence sequences when polls receive \textit{without-replacement} samples from finite populations.

In parliamentary democracies such as India~\cite{rajeeva2002} and the United Kingdom~\cite{payne2003}, individuals in each \textit{constituency} (or \textit{seat})---typically a geographically contiguous region---elect a party based on plurality; the party winning the most seats forms the government. This two-level structure is followed both to elect governments in each state, and for the entire country. Forecasting the winning party in such an \textit{indirect} voting system calls for a more sophisticated sampling procedure. Whereas it would \textit{suffice} to separately identify the winner from each seat by sampling, it might be wasteful to do so when the overall winning party has a clear majority in its number of seats. Rather, one could potentially use the results currently available from \textit{all} the constituencies to decide which ones to query next. 

In this section, we consider a procedure that 
(1) keeps track of the current winners and leaders at the aggregate level, and (2) at each step samples the constituencies that appear most promising to confirm the aggregate trend. In principle, this algorithm, denoted DCB (for ``Difference in Confidence Bounds'') can be coupled with any algorithm that uses confidence bounds for mode estimation. Yet, we obtain the best results when DCB uses PPR-ME as a subroutine, thereby highlighting the relevance of PPR-ME not only as a stopping rule, but also as an input to on-line decision making.

DCB takes cue from the LUCB algorithm for best-arm identification in bandits~\cite{ICML12-shivaram}. At each step $t$, it identifies two parties, $a^{t}$ and $b^{t}$, that appear the most promising to win the overall election: these parties are picked based on their current number of wins and ``leads'' in individual constituencies. Subsequently the algorithm chooses a constituency each for $a^{t}$ and $b^{t}$, samples from which could ``most'' help distinguish the tally of the two. We provide a detailed specification of DCB in Appendix~\ref{app:dcbalgorithm}.

%In this section, we consider the setting of two level elections. In such an election we have several political parties contesting for a national level post such as that of the President or Prime Minister. However individuals vote to elect candidates (from different parties) to represent only their own constituency. The candidate with the most votes is elected at the constituency level, thus here we are left with the task of mode estimation. Our goal however is to predict the winner of the overall election, i.e. the party that wins the most constituencies. 

%In achieving this goal we seek to minimize the number of samples, that is, the number of voters polled. We propose an algorithm called DCB (Difference in Confidence Bounds which tells us which constituency to sample from. We show that it comprehensively outperforms a round robin baseline, i.e., sampling votes from each constituency evenly. The details of the algorithm are given below - 

\vspace{-0.2cm}

\subsection{Performance when Coupled with DCB}
\label{subsec:evaluation}

We compare DCB with a round-robin strategy for picking the next constituency to sample. Both approaches can be implemented with different stopping rules, which are also varied. Table~\ref{tab:elections} shows our results on two recent (and contrasting) elections conducted in India.\footnote{Election results are in the public domain; the authors accessed them at \url{https://www.indiavotes.com/}.} In the 2014 national elections, the winning party secured 282 seats from among 543, giving it a very large victory over the second-place party, which won 44 seats. The second problem instance is from a closer contest in the state of Bihar, in which the top three parties won 80, 71, and 53 seats, of a total 242.


\begin{table}[b]
\vspace{-0.7cm}
\footnotesize
\centering
\scshape
  \caption{Sample complexity of various stopping rules when coupled with (1) round-robin (RR) polling of constituencies and (2) DCB. All experiments are run with mistake probability $\delta=0.01$. Values shown are averages from 10 runs, and show one standard error.  ``Seats resolved'' indicates the number of constituencies in which a winner was identified before the overall procedure terminated.}
  \label{tab:elections}  \begin{tabular}{lccccc}
    
    \toprule
    \multirow{3}{*}{Algorithm} & 
      \multicolumn{2}{c}{India-2014 (543 seats)} &
      \multicolumn{2}{c}{Bihar-2015 (242 seats)} \\
      & \multirow{2}{*}{Samples} & {Seats} & \multirow{2}{*}{Samples} & {Seats}\\
      &  & {Resolved} &  & {Resolved}\\
      \midrule
    % \multirow{2}{*}{$\mathcal{P}_1$: .5, .25 $\times$ 2} & 1vr & 1344$\pm$20 & 444$\pm$14 & 262$\pm$12\\
    %      & 1v1 & 1157$\pm$19 & 346$\pm$13 & 218$\pm$11 \\
    % \multirow{2}{*}{Uniform-PPR} & 1vr & 560815 $\pm$ 7778 & 238 $\pm$ 2 \\
    % & 1v1 & 2054171 $\pm$ 40394 & 221 $\pm$ 1\\
    RR-$\mathcal{A}_1$-1v1 & 1578946 $\pm$ 10255 & 239 $\pm$ 2 & 4201429 $\pm$ 43932  & 221 $\pm$ 1 \\
    RR-$\mathcal{A}_1$-1vr & 1767464 $\pm$ 15828 & 234 $\pm$ 1 & 4841406 $\pm$ 58188 & 222 $\pm$ 1 \\
    RR-KLSN-1v1 & 610181 $\pm$ 7072 & 240 $\pm$ 2 & 2198678 $\pm$ 44514 & 221 $\pm$ 1 \\
    RR-KLSN-1vr & 726512 $\pm$ 6186 & 236 $\pm$ 2 & 2668729 $\pm$ 47535 & 222 $\pm$ 2 \\
    RR-PPR-1v1 & \textbf{471661 $\pm$ 7373} & 241 $\pm$ 3 &\textbf{ 1813213 $\pm$ 42081 }& 221 $\pm$ 1 \\
    RR-PPR-1vr & 560815 $\pm$ 7778 & 238 $\pm$ 2 & 2054171 $\pm$ 40394 & 221 $\pm$ 1 \\\midrule
    DCB-$\mathcal{A}_1$-1v1 & 856678 $\pm$ 3935 & 182 $\pm$ 1 & 2301936 $\pm$ 36399 & 135 $\pm$ 1 \\
    DCB-$\mathcal{A}_1$-1vr & 951684 $\pm$ 5246 & 180 $\pm$ 1 & 2481552 $\pm$ 21483 & 134 $\pm$ 1 \\
    DCB-KLSN-1v1 & 325265 $\pm$ 2096 & 186 $\pm$ 2 & 1127963 $\pm$ 22191 & 139 $\pm$ 2 \\
    DCB-KLSN-1vr & 376108 $\pm$ 4067 & 181 $\pm$ 1 & 1312027 $\pm$ 22892 & 139 $\pm$ 1 \\
    DCB-PPR-1v1 & \textbf{256911 $\pm$ 2096} & 188 $\pm$ 1 & \textbf{883389 $\pm$ 15581} & 142 $\pm$ 2 \\
    DCB-PPR-1vr & 296580 $\pm$ 2372 & 184 $\pm$ 1 & 993495 $\pm$ 18859 & 139 $\pm$ 1 \\
    \bottomrule
  \end{tabular}
%  \vspace{0.1cm}
\normalsize
\end{table}

While it is not the central feature of this paper, it is worth noting that the DCB strategy indeed improves over round-robin polling by roughly a factor of two, regardless of the stopping rule. As intended, it does not waste samples on constituencies that are inconsequential to the overall result (observed in the ``seats resolved'' columns). Of more direct relevance to the theme of the paper is that even when embedded within a decision-making outer loop, PPR continues to outperform $\mathcal{A}_{1}$ and KL-SN, and the 1v1 approach still dominates 1vr.

It must be emphasised that in practice, election surveys typically have the financial budget only for a few thousands of samples, and the time only for a single-stage (non-sequential) poll~\cite{karandikar2018}. Opinion polls must also cope with difficulties in obtaining truthful votes and samples drawn uniformly at random from a population~\cite{paul1979}. We have conveniently assumed a more abstract setting primarily to tease apart the efficiency of different stopping rules for mode estimation. We believe the numerical superiority of PPR-1v1 makes it a good choice for embedding within more complex and realistic models, although we leave the exercise of doing so to future work.

\begin{comment}
\begin{table}[H]
\centering
\scshape
  \begin{tabular}{lccccc}
    
    \toprule
    \multirow{3}{*}{Algorithm} & 
      \multicolumn{2}{c}{India-2014} &
      \multicolumn{2}{c}{Bihar-2015} \\
      & \multirow{2}{*}{Samples} & {Seats} & \multirow{2}{*}{Samples} & {Seats}\\
      &  & {Resolved} &  & {Resolved}\\
      \midrule
    % \multirow{2}{*}{$\mathcal{P}_1$: .5, .25 $\times$ 2} & 1vr & 1344$\pm$20 & 444$\pm$14 & 262$\pm$12\\
    %      & 1v1 & 1157$\pm$19 & 346$\pm$13 & 218$\pm$11 \\
    % \multirow{2}{*}{Uniform-PPR} & 1vr & 560815 $\pm$ 7778 & 238 $\pm$ 2 \\
    % & 1v1 & 2054171 $\pm$ 40394 & 221 $\pm$ 1\\
    Uniform-PPR & 560815 $\pm$ 7778 & 238 $\pm$ 2 & 2054171 $\pm$ 40394 & 221 $\pm$ 1 \\
    Uniform-PPR-ME & 471661 $\pm$ 7373 & 241 $\pm$ 3 & 1813213 $\pm$ 42081 & 221 $\pm$ 1 \\
    Uniform-$\mathcal{A}_1$ & 1767464 $\pm$ 15828 & 234 $\pm$ 1 & 4841406 $\pm$ 58188 & 222 $\pm$ 1 \\
    Uniform-$\mathcal{A}_1$-EVE & 1578946 $\pm$ 10255 & 239 $\pm$ 2 & 4201429 $\pm$ 43932  & 221 $\pm$ 1 \\
    Uniform-KLSN & 726512 $\pm$ 6186 & 236 $\pm$ 2 & 2668729 $\pm$ 47535 & 222 $\pm$ 2 \\
    Uniform-KLSN-EVE & 610181 $\pm$ 7072 & 240 $\pm$ 2 & 2198678 $\pm$ 44514 & 221 $\pm$ 1 \\ \midrule
    DCB-PPR & 296580 $\pm$ 2372 & 184 $\pm$ 1 & 993495 $\pm$ 18859 & 139 $\pm$ 1 \\
    DCB-PPR-ME & 256911 $\pm$ 2096 & 188 $\pm$ 1 & 883389 $\pm$ 15581 & 142 $\pm$ 2 \\
    DCB-$\mathcal{A}_1$ & 951684 $\pm$ 5246 & 180 $\pm$ 1 & 2481552 $\pm$ 21483 & 134 $\pm$ 1 \\
    DCB-$\mathcal{A}_1$-EVE & 856678 $\pm$ 3935 & 182 $\pm$ 1 & 2301936 $\pm$ 36399 & 135 $\pm$ 1 \\
    DCB-KLSN & 376108 $\pm$ 4067 & 181 $\pm$ 1 & 1312027 $\pm$ 22892 & 139 $\pm$ 1 \\
    DCB-KLSN-EVE & 325265 $\pm$ 2096 & 186 $\pm$ 2 & 1127963 $\pm$ 22191 & 139 $\pm$ 2 \\
    \bottomrule
  \end{tabular}
  \caption{Performance of various algorithms in terms of its sample complexity for determining the winner of election when $\delta=0.01$. Seats resolved indicates the number of constituencies in which winner was declared}
\end{table}
\end{comment}

==> NeurIPS submission/sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

We investigate the problem of estimating the mode of a given, arbitrary discrete probability distribution $\mathcal{P} = (p, v, K)$ by observing a sequence of i.i.d. samples drawn according to $\mathcal{P}$. Here $\mathcal{P}$ takes values from the support set $\{v_{1}, v_{2}, \dots, v_{K}\}$ for some $K \geq 2$; for $1 \leq i \leq K$, the probability of obtaining $v_{i}$ from $\mathcal{P}$ is $p_{i}$. We assume that $\mathcal{P}$ has a unique mode, and without loss of generality, $p_{1} > p_{2} \geq p_{3} \geq p_{4} \geq \dots \geq p_{K}$ (which makes $v_{1}$ the mode).

Our aim is to provide a procedure $\mathcal{L}$ to identify the mode of $\mathcal{P}$. At each step $t \geq 1$,
$\mathcal{L}$ can either ask for a sample $x^{t} \sim \mathcal{P}$ or it can terminate and declare its answer. For ``mistake probability'' $\delta \in (0, 1)$, $L$ is said to be $\delta$-correct if for every qualifying discrete distribution $\mathcal{P}$, $L$ terminates with probability $1$ and correctly identifies the mode of $\mathcal{P}$ with probability at least $1 - \delta$. If $\mathcal{L}$ terminates after observing the sequence of samples $x^{1}, x^{2}, \dots, x^{T}$ for some $T \geq 1$, we may assume that its answer is the most frequent value of $\mathcal{P}$ in this sequence, since it can be argued that no other choice can decrease the mistake probability across all problem instances. Hence, it is convenient to view $\mathcal{L}$ simply as a \textit{stopping rule}, which only needs to decide when to terminate. We aim to devise a $\delta$-correct stopping rule $\mathcal{L}$ with low \textit{sample complexity}---informally the number of samples $T$ observed before stopping.


In order to make 
our problem ``properly'' PAC, we could introduce a tolerance parameter $\epsilon$, with the implication that any returned value with associated probability at least $p_{1} - \epsilon$ will be treated as correct. We omit this generalisation, noting that 
it can be handled quite easily by the methods proposed in the paper. In fact, our version with $\epsilon = 0$ exactly matches the problem defined by Shah et al.~\cite{Shah_Choudhury_Karamchandani_Gopalan_2020}, whose algorithms and analysis are our primary baseline. Shah et al.~\cite{Shah_Choudhury_Karamchandani_Gopalan_2020} effectively ``settle'' the PAC mode estimation problem from a theoretical perspective. First they show the following lower bound.
\begin{theorem}[Lower bound~\cite{Shah_Choudhury_Karamchandani_Gopalan_2020}]
\label{thm:lowerbound}
Fix $\delta \in (0, 1)$, $K \geq 2$, and a $\delta$-correct stopping rule $\mathcal{L}$. On each problem instance $\mathcal{P} = (p, v, K)$, the expected number of samples observed by $\mathcal{L}$ is at least $$\frac{p_1}{(p_1-p_2)^2}\ln\left(\frac{1}{2.4\delta}\right).$$
\end{theorem}
They also give a stopping rule, $\mathcal{A}_{1}$, whose sample complexity 
is within a logarithmic factor. 

\begin{theorem}[$\mathcal{A}_{1}$ upper bound~\cite{Shah_Choudhury_Karamchandani_Gopalan_2020}]
\label{thm:a1upperbound}
Fix $\delta \in (0, 1)$, $K \geq 2$, and problem instance $\mathcal{P} = (p, v, K)$. When $\mathcal{A}_{1}$ is run on $\mathcal{P}$, with probability $1 - \delta$, the number of samples it observes is at most $$\frac{592}{3}\frac{p_1}{(p_1-p_2)^2}\ln\left(\frac{592}{3}\sqrt{\frac{K}{\delta}}\frac{p_1}{(p_1-p_2)^2}\right).$$
\end{theorem}
%\jv{k to K in Theorem 2}
In this paper, we approach the PAC mode estimation problem from a different perspective. In recent work, Waudby-Smith and Ramdas~\cite{waudby-ramdas-ppr} propose prior-posterior-ratio (PPR) martingale confidence sequences, a novel framework to obtain ``anytime'' confidence bounds on unknown parameters of a %single-parameter
probability distribution. The resulting stopping rule is simple, with no need for tuning, and yet works surprisingly well in practice, for example to estimate the parameter of a Bernoulli distribution by sampling. Encouraged by this empirical finding, we undertake the generalisation of the PPR martingale test to mode estimation, wherein the $K$-valued input distribution $\mathcal{P}$ has $K - 1$ parameters, for some $K \geq 2$. We denote our generalised stopping rule PPR-ME (PPR applied to mode estimation).

In Section~\ref{sec:pprmcs}, we upper-bound the sample complexity of PPR-ME for the base case of $K = 2$, showing it to be optimal up to a logarithmic factor for the well-studied ``Bernoulli'' setting. This finding might independently bear significance to the push for tighter confidence bounds 
in the bandits literature~\cite{kaufmann2018mixture,Jamieson14}. In Section~\ref{sec:ppr-me}, we describe PPR-ME for $K \geq 2$ and derive an upper bound on its sample complexity. Interestingly, this upper bound also matches the lower bound in Theorem~\ref{thm:lowerbound} up to a logarithmic factor, and marginally improves upon the constant factor in the upper bound from Theorem~\ref{thm:a1upperbound}. In sections \ref{sec:pprmcs} and \ref{sec:ppr-me}, we also provide empirical comparisons between PPR-ME and other approaches to PAC mode estimation. We find strong support for using ``one-versus-one'' comparisons for mode estimation (as in PPR-ME), as opposed to a ``one-versus-rest'' approach (as in $\mathcal{A}_{1}$~\cite{Shah_Choudhury_Karamchandani_Gopalan_2020}).

%Our experimental results, too, make a strong case in favour of PPR-ME.

Over the years, the mode estimation problem has received attention in many different contexts~\cite{Parzen62,Motwani02,Misra82}. We illustrate the gains obtained from PPR-ME in two contrasting real-life applications. In Section~\ref{sec:elections}, we show that PPR-ME, used as a subroutine, can reduce the sample complexity of winner-forecasting in indirect elections~\cite{karandikar2018}. In Section~\ref{sec:blockhains}, we
illustrate the relevance of PPR-ME for
%we show savings on computation for performing
probabilistic verification in permissionless blockchains~\cite{sourav2019}.
%\sj{We don't show savings on computation anymore - mainly lower error}
We conclude with a summary in Section~\ref{sec:conclusion}.


==> NeurIPS submission/sections/ppr-me.tex <==
\section{PPR-ME Stopping Rule for Mode Estimation}
\label{sec:ppr-me}

In this section, we present our generalisation of the PPR-Bernoulli stopping rule to the problem of mode estimation: that is, when the support set is of size $K \geq 2$. In the broader machine learning literature, the most common approaches for generalising $2$-class problems to more classes are ``one-versus-one'' (denoted 1v1) and ``one versus rest'' (denoted 1vr). We investigate both approaches, and present them in turn. Interestingly, we observe overwhelming evidence in favour of using the 1v1 approach for mode estimation. Thus, the PPR-ME stopping rule that we propose based on the investigation in this paper is the same as PPR-1v1, which we describe next.

\subsection{One-versus-one (1v1)  Approach}
\label{subsec:oneversusoneapproach}


In the first $t \geq 1$ samples, let the number of occurrences of value $v_{i}$ be $s_{i}(t)$, $1 \leq i \leq K$. The 1v1 generalisation proceeds based on the idea that if $v_{i}$ is to be declared the mode, we need to be sufficiently sure that $v_{i}$ is more probable than $v_{j}$ for $i, j \in \{1, 2, \dots, K\}, i \neq j$. In keeping, we simultaneously run PPR-Bernoulli tests on each $(i, j)$ pair with mistake probability $\frac{\delta}{K - 1}$. 
Each $(i, j)$ test relies solely on the number of occurrences of $v_{i}$ and $v_{j}$, disregarding other values. Hence it amounts to observing samples from a Bernoulli variable with parameter $\frac{p_{i}}{p_{i} + p_{j}}$, and verifying which side of $\frac{1}{2}$ its mean lies. The overall procedure stops when some $i \in \{1, 2, \dots, K\}$ has won each of its tests. By a union bound, we obtain that with probability at least $1 - \delta$, the (true) mode $v_{1}$ will not ever lose a test. Thus, upon termination,  $v_{1}$ is returned with probability at least $1 - \delta$.
%\sj{Maybe we should mention that a sample is only added to a  pairwise comparison if it belongs to atleast one of the pair}

Whereas the description above suggests we need to monitor $\binom{K}{2}$ tests at each step, closer inspection reveals that a much lighter implementation is possible. As before, let $\text{first}(t)$ denote the index of the most-frequently occurring value (with arbitrary tie-breaking) after $t$ samples: that is, $s^{t}_{\text{first}(t)} \geq s^{t}_{i}$ for $i \in \{1, 2, \dots, K\}$. Now, if at all a winner is identified after $t$ samples, clearly it must be $v_{\text{first}(t)}$, which has as many occurrences as any other value. Hence, we only need to track tests involving $v_{\text{first}(t)}$. Now, it is also immediate that $v_{\text{first}(t)}$ wins all its tests if and only if it defeats the \text{second} most frequently occurring value, which we denote $\text{second}(t)$: that is, 
$\text{second}(t) \in \{1, 2, \dots, K\}, \text{second}(t) \neq \text{first}(t)$ satisfies $s^{t}_{\text{second}(t)} \geq s^{t}_{i}$ for $i \in \{1, 2, \dots, K\} \setminus \{\text{first}(t)\}$. Hence, we may implement our stopping rule, denoted PPR-1v1, using a \textit{single} PPR-Bernoulli test at each step $t \geq 1$.
\begin{center}
\fbox{
\parbox{0.92\textwidth}{
PPR-1v1: 
Stop and declare $v_{\text{first}(t)}$ as mode iff
$\text{Beta}\left(\frac{1}{2}; s^{t}_{\text{first}(t)} + 1, s^{t}_{\text{second}(t)} + 1\right) \leq \frac{\delta}{K - 1}$.
}
}
\end{center}

Whereas a $\Theta(K)$ initialisation step is needed to initialise all counts to zero, observe that the computation needed at each step $t \geq 1$ is only $\Theta(1)$---which suffices for identifying $\text{first}(t)$ and
$\text{second}(t)$ based on their previous values, and incrementing the count of the $x_{t}$. Interestingly, we are able to show a sample complexity upper bound for this simple procedure to improve upon the one from Theorem~\ref{thm:a1upperbound}~\cite{Shah_Choudhury_Karamchandani_Gopalan_2020}, albeit by a small constant factor.

\begin{theorem}[PPR-1v1 upper bound]
\label{thm:ppr-meupperbound}
Fix $\delta \in (0, 1)$, $K \geq 2$, and problem instance $\mathcal{P} = (p, v, K)$. When PPR-ME is run on $\mathcal{P}$, with probability $1 - \delta$, the number of samples it observes is at most $$t^{\star} = \frac{194.07p_1}{(p_1-p_2)^2}\ln\left(\sqrt{\frac{79.68(K-1)}{\delta}}\frac{p_1}{(p_1-p_2)}\right).$$
\end{theorem}
\begin{proof}
Fix arbitrary $t > t^{\star}$ and $j \geq 2$. Our strategy is to show that with sufficiently high probability, $v_{1}$ and $v_{j}$ will have separated before $t$ pulls.  First, let $Z_{t}$ denote the sum of the number of occurrences of $v_{1}$ and $v_{j}$ in the first $t$ samples: that is, $Z^{t} = s^{t}_{1} + s^{t}_{j}$. Clearly $Z_{t}$ is a binomial random variable with parameters $t$ and $(p_{1} + p_{j})$, We argue that $Z^{t}$ cannot fall too far below its mean. Concretely, take $\delta^{\prime} = \frac{\delta}{2 (K - 1)}$ and $l = \sqrt{\frac{2 \ln(\frac{1}{\delta^{\prime}})}{(p_{1} + p_{2})t}}$. A Chernoff bound yields
$$\mathbb{P}\{Z_{t} \leq (1 - l) (p_{1} + p_{j}) t \} \leq \exp\left(-\frac{l^{2}(p_{1} + p_{j})t}{2}\right) \leq \delta^{\prime}$$
for our choice of $l$. Thus, with probability at least $1 - \delta^{\prime}$, $v_{1}$ and $v_{j}$ together have more than $(1 - l) (p_{1} + p_{j}) t$ samples. Now, the test to separate $v_{1}$ and $v_{j}$ is PPR-Bernoulli on a Bernoulli variable with parameter $q_{1} = \frac{p_{1}}{p_{1} + p_{j}} > \frac{1}{2}$. Although PPR-ME runs this test with mistake probability $\frac{\delta}{K - 1}$, imagine running it with mistake probability $\delta^{\prime} = \frac{\delta}{2(K - 1)}$. The latter test would necessarily incur equal or more samples on \textit{every} run. Yet, from Lemma~\ref{lem:ppr-bernoulli-upperbound}, we know that with probability at least $1 - \delta^{\prime}$, the latter will terminate after at most $u = \frac{20.775 q_1}{(q_1-\frac{1}{2})^2}\ln\left(\frac{2.49}{(q_1-\frac{1}{2})^2 \delta^{\prime}}\right)$ samples. It can be verified that for $t > t^{\star}$, $u < (1 - l)(p_{1} + p_{j})t$ (calculation shown in Appendix~\ref{app:calculationinproofoftheorempprmeupperbound}). In other words, the probability that $v_{1}$ and $v_{j}$ have \textit{not} separated before $t$ pulls is at most $2\delta^{\prime}$.

Since the argument above holds for arbitrary $j \geq 2$, a union bound establishes that with probability at least $1 - \delta$, $v_{1}$ must have separated from all other values---implying termination---before $t$ pulls.
\end{proof}

\subsection{One-versus-rest (1vr) Approach}
\label{subsec:oneversusrestapproach}
Notice that under PPR-1v1, sample $x^{t}$ at each step $t \geq 1$ contributes to only $K - 1$ tests;
$\binom{K - 1}{2}$ tests corresponding to values other than $x^{t}$ receive no information. The 1vr approach becomes an alternative to address this \textit{apparent} wastage of information. Under the 1vr scheme, we associate a Bernoulli variable $B_{i}$ with each value $v_{i}$, $1 \leq i \leq K$, which has probability $p_{i}$ of generating $v_{i}$, and probability $1 - p_{i}$ of generating its \textit{negation} ``$\neg v_{i}$''. Consequently, each sample of $\mathcal{P}$ adds to one of the outcomes of $B_{i}$ for \textit{each} $i \in \{1, 2, \dots, K\}$. We draw an anytime confidence sequence for $B_{i}$ with mistake probability $\frac{\delta}{K}$, and terminate after $t \geq 1$ samples if the confidence set of $B_{\text{first}(t)}$ does not overlap with any of the others. Invoking the PPR martingale confidence sequence, we note that 
with probability at least $1 - \frac{\delta}{K}$, $p_{i}$ will lie  in all the intervals $(\text{LCB}^{t}_{i}, \text{UCB}^{t}_{i})$, $t \geq 1$, where
\begin{equation*}
    \text{LCB}^{t}_{i} = \min \left\{\hat{p} \in [0, 1]: \pi^{t}(\hat{p}) = \frac{\delta}{K} \right\} \text{  and  } \text{UCB}^{t}_{i} = \max \left\{\hat{p} \in [0, 1]: \pi^{t}(\hat{p}) = \frac{\delta}{K} \right\}
\end{equation*}
can be computed numerically. The $\delta$-correctness of the 1vr rule, summarised below, is established by applying a union bound on the mistake probabilities of each $B_{i}$, $1 \leq i \leq K$.
%\jv{define PPR-EVR here}
\begin{center}
\fbox{
\parbox{0.95\textwidth}{
PPR-1vr: 
Stop and declare $v_{\text{first}(t)}$ as mode iff for $1 \leq i \leq K$, $i \neq \text{first}(t)$, 
$\text{LCB}^{t}_{\text{first}(t)} \geq \text{UCB}^{t}_{i}.$
}
}
\end{center}
%\sj{This is not the stopping rule we use - we stop if $LCB^t(first) > UCB^t(k)$ for all $k \neq first$. This is because we don't have a proof maintaining top $2$ is enough here.}

\subsection{Empirical Comparisons with other Stopping Rules for Mode Estimation}
\label{subsec:empiricalcomparisonmodeestimation}

The $\mathcal{A}_{1}$ algorithm of Shah et al.~\cite{Shah_Choudhury_Karamchandani_Gopalan_2020} is essentially a 1vr approach that uses Empirical Bernstein confidence bounds~\cite{maurer2009}. Noting that it can just as well be implemented in a 1v1 form, we include such a variant, denoted $\mathcal{A}_{1}$-1v1, in our experimental comparisons with PPR. For good measure, we also include 1v1 and 1vr variants based on the KL-SN confidence bound~\cite{garivier2013}, which finished second to PPR-Bernoulli for $K = 2$ (see Section~\ref{sec:pprmcs}). Table \ref{tab:tab_multiK} shows the performance of 1v1 and 1vr versions of PPR, $\mathcal{A}_{1}$, and KL-SN on a variety of distributions. We observe the same trend on \textit{each} problem instance: (1) The 1v1 variant of each stopping rule outperforms the corresponding 1vr variant, and (2) PPR is most sample-efficient, followed by KL-SN and $\mathcal{A}_{1}$. In line with the upper bound from theorems~\ref{thm:a1upperbound} and \ref{thm:ppr-meupperbound}, it does appear that the sample complexity is largely determined by $p_{1}$ and $p_{2}$ (identical for instances $\mathcal{P}_{5}$ and $\mathcal{P}_{6}$) in the table. The logarithmic dependence on $K$ results in a slightly larger number of samples for all these methods on $\mathcal{P}_{6}$.
% \vspace{-0.5cm}
\begin{table}[b]
\footnotesize
    \centering
    \scshape
\caption{Sample complexity comparison for mode estimation, run with mistake probability $\delta = 0.01$. The number after the $\times$ symbol indicates the multiplicity of that particular probability value in the distribution; thus $\mathcal{P}_{1}$ has $p = (0.5, 0.25, 0.25)$. The values reported are averages from 100 or more runs, and show one standard error.}
% \caption{Sample complexity comparison for mode estimation, run with mistake probability $\delta = 0.01$. The number after the $\times$ symbol indicates the multiplicity of that particular probability value in the distribution; thus $\mathcal{P}_{1}$ has $p = (0.5, 0.25. 025)$. The values reported in this and the forthcoming table are averages from \textcolor{red}{100-200} runs, and show one standard error. \textcolor{red}{Include $K$ as a column in between distribution and type. What?--did P6 and P7 give exactly the same numbers for all the methods, or did you copy the wrong row in?} \sj{Yes, they give the same answer due to identical samples coming in for top 2 parties - same random seed} }
        \label{tab:tab_multiK}
    \begin{tabular}{l c c c c c}
    \hline
    \toprule
        Distribution & K & Type & $\mathcal{A}_{1}$ \cite{Shah_Choudhury_Karamchandani_Gopalan_2020} & KL-SN \cite{garivier2013}  & PPR \\
        \midrule
        \multirow{2}{*}{$\mathcal{P}_1$: .5, .25 $\times$ 2} & \multirow{2}{*}{3} & 1vr & 1344$\pm$20 & 444$\pm$14 & 262$\pm$12\\
         & & 1v1 & 1157$\pm$19 & 346$\pm$13 & \textbf{218$\pm$11} \\
         \midrule \multirow{2}{*}{$\mathcal{P}_2$: .4, .2 $\times$ 3} & \multirow{2}{*}{4} & 1vr & 1919$\pm$29 & 662$\pm$18 & 397$\pm$15\\
         & & 1v1 & 1515$\pm$25 & 472$\pm$15 & \textbf{298$\pm$13}\\
         \midrule \multirow{2}{*}{$\mathcal{P}_3$: .2, .1 $\times$ 8} & \multirow{2}{*}{9} & 1vr & 5082$\pm$51 & 3767$\pm$68 & 1201$\pm$29\\
         & & 1v1 & 3340$\pm$43 & 1138$\pm$32 & \textbf{789$\pm$28}\\
         \midrule \multirow{2}{*}{$\mathcal{P}_4$: {.1, .05 $\times$ 18 }} & \multirow{2}{*}{19} & 1vr & 12014$\pm$129 & 4540$\pm$80 & 2850$\pm$55\\
         & & 1v1 & 7351$\pm$88 & 2554$\pm$56 & \textbf{1840$\pm$53}\\
         \midrule \multirow{2}{*}{$\mathcal{P}_5$: {.35, .33, .12, .1 $\times$ 2}} & \multirow{2}{*}{5} & 1vr & 155277$\pm$2356 & 63739$\pm$2238 & 38001$\pm$1311\\
         & & 1v1 & 117988$\pm$2078 & 47205$\pm$1291 & \textbf{33660$\pm$1125}\\
         \midrule 
         
         %\multirow{2}{*}{$\mathcal{P}_6$: {.35, .33, .2, .07, .05}} & \multirow{2}{*}{5} & 1vr & 155277$\pm$2356 & 63739$\pm$2238 & 38001$\pm$1311\\
         %& & 1v1 & 117988$\pm$2078 & 47954$\pm$1876 & 33660$\pm$1125\\
         %\midrule
         
         \multirow{2}{*}{$\mathcal{P}_6$: {.35, .33,  .04 $\times$ 8}} & \multirow{2}{*}{10} & 1vr & 158254$\pm$2442 & 66939$\pm$2241 & 41963$\pm$1330\\
         & & 1v1 & 121150$\pm$2183 & 49576$\pm$1341 & \textbf{36693$\pm$1185}\\
    %   $\mathcal{P}_7$: .35, .33,  .04 $\times$ 8 & 158254$\pm$2442 & 121150$\pm$2183 &a$\pm$b &50942$\pm$1947 & 41963$\pm$1330 & 36693$\pm$1185 \\
        % \hline
        % \midrule
        \bottomrule
        \end{tabular}
%        \vspace{0.1cm}
\normalsize
    \end{table}

%key things to note include looking at the performance when the number of parties $K$ is large when $K=19$ as in the 4th row. The last 3 rows consider the situation where $p_1$ and $p_2$ are very close to each other. Rows 5 and 6 show that the sample complexity depends only on $p_1$ and $p_2$ as the number of samples are very close to each other which corrobates the claim made earlier. The last row has the same $p_1$ and $p_2$ but with a larger $K$ which increases the number of samples due to a $K$ in the log factor.  

Interestingly, not only do the 1v1 variants of each method perform better than 1vr in aggregate, we observe that they terminate \textit{before} the 1vr variants on \textit{every} single run. Intuitively, it appears that although the 1vr variants update all their $K$ tests with each sample, the condition to separate any two variables becomes weaker than that under the corresponding 1v1 variant. We discuss this effect in Appendix~\ref{app:relatingpprmeterminationandpprevrtermination}. It is also worth noting that PPR-1v1, which can be implemented with a constant number of arithmetic operations, is \textit{computationally} the fastest among the methods presented in this section. 

%Before proceeding,  it is also worth noting that the 1v1 approach for mode estimation can easily be generalised to ``top $m$ selection''~\cite{Shah_Choudhury_Karamchandani_Gopalan_2020} by comparing the $m$-th and $(m + 1)$-st values rather than the first and the second, with a reduced mistake probability.



%The results are shown in Figure \ref{fig:fig_binary} which show that using confidence sequences based PPR outperforms all other baselines in the $K = 2$ case. We next compare the stopping rules for $K > 2$ for a variety of distributions as shown in Table \ref{tab:tab_multiK}. The number after the $\times$ symbol indicates the multiplicity of that particular probability value in the distribution. Some key things to note include looking at the performance when the number of parties $K$ is large when $K=19$ as in the 4th row. The last 3 rows consider the situation where $p_1$ and $p_2$ are very close to each other. Rows 5 and 6 show that the sample complexity depends only on $p_1$ and $p_2$ as the number of samples are very close to each other which corrobates the claim made earlier. The last row has the same $p_1$ and $p_2$ but with a larger $K$ which increases the number of samples due to a $K$ in the log factor.  \\
\begin{comment}
\sj{We note the average runtimes of the algorithms across 10 runs on the distribution $\mathcal{P}_7$ on an Intel(R) Core(TM) i7-8750H CPU @ 2.20GHz Processor (all in seconds):\\
PPR-ME: 1.34 +- 0.15 \\
SE-EVE: 6.36 +- 0.38 \\
SE: 8.09 +- 0.50 \\
KL-SN EVE: 16.92 +- 1.88 \\
PPR-EVR: 51.61 +- 6.96 \\
KL-SN: 162 +- 16 \\
This shows that PPR-1v1 is about $5x$ faster than it's nearest competitor in terms of runtime. The nearest competitor in terms of sample complexity is PPR-1vr, which takes more than $35$ times the amount of time taken by PPR-1v1. Detailed results are given in Appendix~\ref{CodeAppendix}. \\\\
Updated values for 100 iterations for fastest 2 methods, and least sample complexity methods:\\
PPR-ME: 1.28 +- 0.06 \\
SE-EVE: 6.65 +- 0.17 \\
PPR: 51.50 +- 2.37 \\
Illustrate speed of PPR-ME. Write your own beta function, don't use inbuilt - 5x speedup. 
}
\end{comment}


\begin{comment}
$$\text{Beta}(\frac{1}{2}; \alpha, \beta + 1) \leq \delta \implies \text{Beta}(\frac{1}{2}; \alpha, \beta) \leq \delta.$$

It suffices to show that $\text{Beta}(\frac{1}{2}; \alpha, \beta + 1) \geq  \text{Beta}(\frac{1}{2}; \alpha, \beta)$ which can be shown simply by writing the definition of the beta pdf as shown below:

$$ \frac{\left (\frac{1}{2}\right ) ^{(\alpha+\beta+1)} (\alpha + \beta)!}{(\alpha-1)!\beta!} \geq \frac{\left (\frac{1}{2}\right ) ^{(\alpha+\beta)} (\alpha + \beta-1)!}{(\alpha-1)!(\beta-1)!} $$

$$  \frac{\alpha+\beta}{2\beta} \geq 1 \text{ which is true when } \alpha \geq \beta  $$
This concludes our claim that if the confidence sequences of the top two parties are disjoint, we can claim that the first party will have it's confidence sequence disjointed with all other remaining parties.


\end{comment}


==> NeurIPS submission/sections/ppr2party_proof.tex <==
\subsection{Constant factor tightening}

We solve the special case of 2 parties. Suppose our parameters are $p, 1-p$, with $p > 0.5$. If the confidence sequences of both the parameters don't contain $\frac{1}{2}$ and the iteration is a successful one (i.e, CS for $p$ contains $p$ and CS for $1-p$ contains $1-p$), then we can be sure that if $\frac{1}{2}$ is not contained in the confidence sequence of both parameters, then we are done. In two parties, we only need maintain one confidence sequence, since the other is simply a mirror image. We compute the probability of $\frac{1}{2}$ not being present in the CS as follows: (note that $\theta^*$ is the parameter for the CS, i.e $\theta^* = p$)
\begin{gather*}
    \mathbb{P}\left(R_t(\theta) > \frac{1}{\delta}\right) = \int_{X_1^t}\mathds{1}\left\{R_t(\theta) > \frac{1}{\delta}\right\} P_{\theta^*}(X_1^t)dX_1^t, \theta = \frac{1}{2}
\end{gather*}
We will compute the above for a general $\theta \in [0, 1]$ and substitute our specific value of $\theta = \frac{1}{2}$ later. $X_1^t$ denotes an instance of 0-1 sequence of observations. The expression inside the indicator random variable can be simplified to obtain the following:
\begin{align*}
    \mathds{1}\left\{R_t(\theta) > \frac{1}{\delta}\right\} = \mathds{1}\left\{\frac{1}{\pi_t(\theta)} > \frac{1}{\delta}\right\} = \mathds{1}\left\{\frac{\int P_{\eta}(X_1^t)d\eta}{P_\theta(X_1^t)} > \frac{1}{\delta}\right\}
\end{align*}
\rs{Should be capital X in the denominator} \sj{Fixed}\\

The integral inside the indicator function is independent of the position of 0-1 outcomes within the sequence $X_1^t$ and it only depends on the number of zeros and ones in the instance. Suppose we consider the instances which contain $k$ ones; then, we have
\begin{align*}
    \mathds{1}\left\{R_t(\theta) > \frac{1}{\delta}\right\} = \mathds{1}\left\{\delta > \frac{(t + 1)!}{k!(t-k)!}\theta^k (1 - \theta)^{t - k}\right\}
\end{align*}
From the above equations, we derive the exact expression for $\mathbb{P}(R_t(\frac{1}{2}) > \frac{1}{\alpha})$:
\begin{gather*}
    \mathbb{P}\left(R_t\left(\frac{1}{2}\right) > \frac{1}{\delta}\right) = \sum_{k=0}^t \binom{t}{k} \theta^{*k} (1 - \theta^*)^{t-k}\mathds{1}\left\{\delta > \frac{(t + 1)!}{k!(t-k)!}2^{-t}\right\}
\end{gather*}
We now break the expression into two parts.
\begin{align*}
    \mathbb{P}\left(R_t\left(\frac{1}{2}\right) > \frac{1}{\delta}\right) &= \sum_{k=0}^t \binom{t}{k} \theta^{*k} (1 - \theta^*)^{t-k}\mathds{1}\left\{\delta > \frac{(t + 1)!}{k!(t-k)!}2^{-t}\right\}\\
    = &\sum_{k=0}^{\frac{t}{2}} \binom{t}{k} \theta^{*k} (1 - \theta^*)^{t-k}\mathds{1}\left\{\frac{\delta}{t + 1} > \binom{t}{k}2^{-t}\right\} + \\
    &\sum_{k=\frac{t}{2} + 1}^{t} \binom{t}{k} \theta^{*k} (1 - \theta^*)^{t-k}\mathds{1}\left\{\frac{\delta}{t + 1} > \binom{t}{t - k}2^{-t}\right\}
\end{align*}
\rs{floor(t/2) instead of t/2}
We have split the summation in this manner as it allows to use the following inequality for the binomial coefficients inside the indicator function.
\begin{equation*}
    \binom{t}{\alpha t} \leq 2^{tH_b(\alpha)}\,\, \text{where $t \in \mathbb{N}$ and $\alpha \in \left[0, \frac{1}{2}\right]$}
\end{equation*}
\rs{Haven't verified this inequality, should add reference}
\sj{Reference: https://arxiv.org/pdf/1406.7872.pdf}
The definition of binary entropy function $H_b$ for $p \in [0, 1]$:
\begin{equation*}
    H_b(p) = 
    \begin{dcases}
    0 & p \in \{0, 1\}\\
    -p\log_2p - (1 - p)\log_2(1 - p) & \text{otherwise}\\
    \end{dcases}
\end{equation*}
Invoking this inequality in the probability expression, we arrive at the lower bound:
\begin{align*}
    \mathbb{P}\left(R_t\left(\frac{1}{2}\right) > \frac{1}{\delta}\right) \geq  &\sum_{k=0}^{\frac{t}{2}} \binom{t}{k} \theta^{*k} (1 - \theta^*)^{t-k}\mathds{1}\left\{\frac{1}{t}\log_2\left(\frac{\delta}{t + 1}\right) + 1 > H_b\left(\frac{k}{t}\right)\right\} + \\
    &\sum_{k=\frac{t}{2} + 1}^{t} \binom{t}{k} \theta^{*k} (1 - \theta^*)^{t-k}\mathds{1}\left\{\frac{1}{t}\log_2\left(\frac{\delta}{t + 1}\right) + 1 > H_b\left(\frac{t - k}{t}\right)\right\}
\end{align*}
Using the fact that:
\[H_b(p) \leq 2\sqrt{p(1 - p)} \,\,\text{if}\,\, p \leq \frac{1}{2} \]
\rs{Haven't verified this}
\sj{Reference - https://math.stackexchange.com/questions/1432043/an-upper-bound-of-binary-entropy}
The summation is further lower-bounded by:
\begin{align*}
    \mathbb{P}\left(R_t\left(\frac{1}{2}\right) > \frac{1}{\delta}\right) \geq  &\sum_{k=0}^{t} \binom{t}{k} \theta^{*k} (1 - \theta^*)^{t-k}\mathds{1}\left\{\frac{1}{2}\left[\log_2\left(\frac{\delta}{t + 1}\right) + t\right] > \sqrt{k(t - k)}\right\}
\end{align*}
\rs{The LHS in the indicator in the first equation should be positive} \sj{Should add a note here that this holds for the t we consider}
The range of $k$ which satisfies the condition inside the indicator function is:
\[k \in \left[0, \frac{t - \sqrt{t^2 - 4\beta^2}}{2}\right) \bigcup \left(\frac{t + \sqrt{t^2 - 4\beta^2}}{2}, t\right] \,\, \text{where} \,\, \beta = \frac{1}{2}\left[\log_2\left(\frac{\delta}{t + 1}\right) + t\right]\] 
Slightly loosening this bound, we get
\begin{align*}
    k \in \left[0, \frac{t - \sqrt{2t\log_2\left(\frac{t+1}{\delta}\right)}}{2}\right) \bigcup \left(\frac{t + \sqrt{2t\log_2\left(\frac{t+1}{\delta}\right)}}{2}, t\right]
\end{align*}
So, we have a range of $k$ values. Let this range be $K$. We will lower bound the probability of $\sum_{i:K}\theta^{*i}(1-\theta^*)^{t-i}$ by $1-\delta$, and thus find the values of $t$ satisfying this equation. To that end, we use Theorem 2.1 of `Five Proofs of Chernoff's Bound with Applications' \cite{mulzer2019proofs} to bound the tail probability for a binomial random variable, which states
\begin{gather*}
    \mathbb{P}(H(t) \geq (\theta^*+\epsilon)t) \leq e^{-D_{KL} (\theta^*+\epsilon || \theta^*)t } \\
    \mathbb{P}(H(t) \leq (\theta^*-\epsilon)t) \leq e^{-D_{KL} (\theta^*-\epsilon || \theta^*)t }
\end{gather*}
Using this in our case considering $H(t)$ as a binomial random variable, we get

\begin{gather*}
    \sum_{k=(\theta^*-\epsilon)t}^{(\theta^* +\epsilon)t} \binom{t}{k} \theta^{*k} (1 - \theta^*)^{t-k} = \mathbb{P}\left(\left(\theta^*-\epsilon\right)t \leq H(t)  \leq \left(\theta^*+\epsilon\right)t\right) \\ \geq  1 - e^{-D_{KL} (\theta^*+\epsilon || \theta^*)t }  - e^{-D_{KL} (\theta^*-\epsilon || \theta^*)t }  \\
    \implies \mathbb{P}\left(R_t\left(\frac{1}{2}\right) \leq \frac{1}{\delta} \right) \leq e^{-D_{KL} (\theta^*+\epsilon || \theta^*)t }  + e^{-D_{KL} (\theta^*-\epsilon || \theta^*)t }
\end{gather*}
\rs{We can exclude the $\theta^*$ + $\epsilon$ term}
We want $\mathbb{P}\left(R_t\left(\frac{1}{2}\right) > \frac{1}{\alpha}\right) \geq 1 - \alpha$. A sufficient condition for the above to hold is
\begin{gather*}
    \max \left( e^{-D_{KL} (\theta^*+\epsilon || \theta^*)t }  , e^{-D_{KL} (\theta^*-\epsilon || \theta^*)t } \right) \leq \frac{\alpha}{2} \\
    \implies t * \min(D_{KL} (\theta^*+\epsilon || \theta^*), D_{KL} (\theta^*-\epsilon || \theta^*)) \geq \ln\left(\frac{2}{\alpha}\right) 
\end{gather*}

\sj{I've added an analytical proof for the KL divergence claim below; removed the plot.}

We note that $\theta^* > \frac{1}{2}$. \\
\textbf{Lemma}: $KL(c+y, c) \geq KL(c-y, c)$, $c > 0.5, y \leq 1-c$. \\\\
\textbf{Proof}: We want to show that 
\begin{gather*}
    KL(c+y, c) \geq KL(c-y, c), c > 0.5, y \leq 1-c \\
    \Leftrightarrow (c+y)\log\left(\frac{c+y}{c}\right)+(1-c-y)\log\left(\frac{1-c-y}{c}\right) \geq (c-y)\log\left(\frac{c-y}{c}\right)+(1-c+y)\log\left(\frac{1-c+y}{c}\right) \\
    \Leftrightarrow (c+y)\log(c+y) + (1-c-y)\log(1-c-y) \geq (c-y)\log(c-y) + (1-c+y)\log(1-c+y)
\end{gather*}
Let 
\begin{gather*}
    f(y) = (c+y)\log(c+y)+(1-c-y)\log(1-c-y)-(c-y)\log(c-y)-(1-c+y)\log(1-c+y) \\
    f'(y) = \log\left(\frac{(c+y)(c-y)}{(1-c+y)(1-c-y)}\right) \\
    c \geq 1-c \implies \frac{c^2-y^2}{(1-c)^2-y^2} \geq 1 \implies \log\left(\frac{(c+y)(c-y)}{(1-c+y)(1-c-y)}\right) \geq 0 \\
    \implies f'(y) \geq 0
\end{gather*}
Thus, we showed that $f'(y) \geq 0$. Since $f(0) = 0$, thus $f(y) \geq 0 \: \forall \: y \in \left[0, 1-c\right]$.

Thus, we are left with the sufficient condition for $t$ as 
\begin{gather*}
    t * D_{KL}(\theta^*-\epsilon || \theta^*) \geq \ln\left(\frac{2}{\alpha}\right),\\ 
    \epsilon = \theta^* - \frac{1}{2}\left(1 + \sqrt{\frac{2\log_2\left(\frac{t+1}{\delta}\right)}{t}} \right), \epsilon \geq 0
\end{gather*}
We will note that $\epsilon \geq 0$ holds later. For now, we try to find stronger sufficient conditions on $t$. To that end, we use that 
\begin{gather*}
    D_{KL}(x, y) \geq \frac{(x-y)^2}{2y}, x \leq y\\
    \implies D_{KL}\left(\theta^*-\epsilon, \theta^*\right) \geq \frac{\epsilon^2}{2\theta^*}
\end{gather*}

\sj{Current reference: https://en.wikipedia.org/wiki/Chernoff\_bound. Better reference to be found}

So, a sufficient condition for 
\begin{gather*}
    t * D_{KL}(\theta^*-\epsilon || \theta^*) \geq \ln\left(\frac{2}{\alpha}\right)
\end{gather*}
is given as
\begin{gather*}
    \frac{t\epsilon^2}{2\theta^*} \geq \ln\left(\frac{2}{\alpha}\right) \\
    \implies t \geq \frac{2\theta^*}{\epsilon^2}\ln\left(\frac{2}{\alpha}\right)
\end{gather*}
To find a sufficient condition for $t$ to satisfy the above, we can find a lower bound on $\epsilon^2$ and use it in the expression above. We have 
\begin{gather*}
    \epsilon^2 =  \left(\left(\theta^*-\frac{1}{2}\right) -\sqrt{\frac{\log_2\left(\frac{t+1}{\delta}\right)}{2t}} \right)^2\\
    \epsilon^2 = \left(\theta^*-\frac{1}{2}\right)^2 + \frac{\log_2\left(\frac{t+1}{\delta}\right)}{2t} - 2\left(\theta^*-\frac{1}{2}\right)\sqrt{\frac{\log_2\left(\frac{t+1}{\delta}\right)}{2t}}\\
    \implies \epsilon^2 \geq \left(\theta^*-\frac{1}{2}\right)^2 - 2\left(\theta^*-\frac{1}{2}\right)\sqrt{\frac{\log_2\left(\frac{t+1}{\delta}\right)}{2t}}
\end{gather*}
Consider two cases: $\theta^* \leq 0.6, \theta^* > 0.6$. \\
\rs{Should this be $\theta^*$ instead of $\theta$} \\
\textbf{Case 1: $\theta^* \leq 0.6$} \\
We will find a sufficient condition on $t$ for the fact that 
\begin{gather*}
    \frac{t}{C_1}\left(\theta^*-\frac{1}{2}\right)^2 \geq \log_2\left(\frac{t+1}{\delta}\right)
\end{gather*}
where $C_1 = 2.4488$.\\
We find a sufficient $t$ such that 
\begin{gather*}
    \frac{t}{C_1}\left(\theta^*-\frac{1}{2}\right)^2 \geq \log_2\left(\frac{t+1}{\delta}\right) \\ 
    \implies t \geq \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{t+1}{\delta}\right)
\end{gather*}
We let $t$ be of the form
\begin{gather*}
    t = \frac{C_1C_2}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right),
\end{gather*}
where $C_2$ is a constant. \\
Note that, for this choice of $t$, (We will show later that $t \geq 4000$ is also true for the first line to hold)
\begin{gather*}
    t+1 \leq 1.00025t \\ 
    \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{t+1}{\delta}\right) \leq \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{1.00025t}{\delta}\right) \\
    \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{t+1}{\delta}\right) \leq \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2(1.00025C_2) + 0.3839\frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{C_1}{(\theta-\frac{1}{2})^2\delta}\right) + \\ \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)
\end{gather*}
where the last step is true because
\begin{gather*}
    \log_2\left(\log_2\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)\right) \leq 0.3839\log_2\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)
\end{gather*}
where we used that, for $x \geq 200$, 
\begin{gather*}
    \log_2\left(\log_2\left(x\right)\right) \leq 0.3839\log_2\left(x\right)
\end{gather*}
Thus, we get 
\begin{gather*}
    \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{t+1}{\delta}\right) \leq \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)\left(1.3839+\log_2\left(1.00025C_2\right)\right) \leq \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)C_2
\end{gather*}
where the last step is true when $C_2 = 2.9402$. Thus,
\begin{gather*}
    t = \frac{2C_1C_2\theta^*}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)
    \implies t = \frac{C_3\theta^*}{(\theta^*-\frac{1}{2})^2}\ln\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right),
\end{gather*}
where $C_3 = 20.775 \geq 2C_1C_2\log_2(e)$
satisfies the above inequality. \\\\
So now, if the condition on $t$ is satisfied, we have
\begin{gather*}
    \epsilon^2 \geq \left(\theta^*-\frac{1}{2}\right)^2 - 2\left(\theta^*-\frac{1}{2}\right)\sqrt{\frac{\log_2\left(\frac{t+1}{\delta}\right)}{2t}} \geq \left(\theta^*-\frac{1}{2}\right)^2 - 2\left(\theta^*-\frac{1}{2}\right)\frac{\left(\theta^*-\frac{1}{2}\right)}{2.21305}\\
    \implies \epsilon^2 \geq C_4\left(\theta^*-\frac{1}{2}\right)^2,
\end{gather*}
where $C_4 = 0.09627$.\\
Previously, we had remarked that it was sufficient to have
\begin{gather*}
    t \geq \frac{2\theta^*}{\epsilon^2}\ln\left(\frac{2}{\alpha}\right)
\end{gather*}
We can loosen this by using the lower bound on $\epsilon$ to: it is sufficient to satisfy
\begin{gather*}
    t \geq \frac{C_5\theta^*}{\left(\theta^*-\frac{1}{2}\right)^2}\ln\left(\frac{2}{\alpha}\right),
\end{gather*}
where $C_5 = 20.775$. \\
To make both the lower bound on $\epsilon$ and the above equation valid, we note that the following choice of $t$ works:
\begin{gather*}
    t = \frac{C_5\theta^*}{\left(\theta^*-\frac{1}{2}\right)^2}\max\left(\left(\ln\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right), \ln\left(\frac{2}{\alpha}\right)\right)\right)
\end{gather*}
We note that, when $\alpha = \delta$, this leaves us with the following choice of $t$:

\begin{gather*}
    t = \frac{20.775\theta^*}{\left(\theta^*-\frac{1}{2}\right)^2}\left(\ln\left(\frac{2.45}{(\theta^*-\frac{1}{2})^2\delta}\right)\right)
\end{gather*}
Note that $t \geq 4000$, since $\theta \leq 0.6$.\\\\\\

\textbf{Case 2: $\theta^* > 0.6$}
We will find a sufficient condition on $t$ for the fact that 
\begin{gather*}
    \frac{t}{C_1}\left(\theta^*-\frac{1}{2}\right)^2 \geq \log_2\left(\frac{t+1}{\delta}\right)
\end{gather*}
where $C_1 = 2.4877$.\\
We find a sufficient $t$ such that 
\begin{gather*}
    \frac{t}{C_1}\left(\theta^*-\frac{1}{2}\right)^2 \geq \log_2\left(\frac{t+1}{\delta}\right) \\ 
    \implies t \geq \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{t+1}{\delta}\right)
\end{gather*}
We let $t$ be of the form
\begin{gather*}
    t = \frac{C_1C_2}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right),
\end{gather*}
where $C_2$ is a constant. \\
Note that, for this choice of $t$, (We will show later that $t \geq 100$ is also true for the first line to hold)
\begin{gather*}
    t+1 \leq 1.01t \\ 
    \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{t+1}{\delta}\right) \leq \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{1.01t}{\delta}\right) \\
    \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{t+1}{\delta}\right) \leq \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2(1.01C_2) + 0.5228\frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{C_1}{(\theta-\frac{1}{2})^2\delta}\right) + \\ \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)
\end{gather*}
where the last step is true because
\begin{gather*}
    \log_2\left(\log_2\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)\right) \leq 0.5228\log_2\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)
\end{gather*}
where we used that, for $x \geq 9.64$, 
\begin{gather*}
    log_2\left(\log_2\left((x\right)\right) \leq 0.5228\log_2\left(x\right)
\end{gather*}
\rs{Think there's one extra log in the LHS} 
\sj{Fixed}\\
Thus, we get 
\begin{gather*}
    \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{t+1}{\delta}\right) \leq \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)\left(1.5228+\log_2\left(1.01C_2\right)\right) \leq \frac{C_1}{(\theta^*-\frac{1}{2})^2}\log\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)C_2
\end{gather*}
where the last step is true when $C_2 = 3.228$. Thus, using that $\theta > 0.6$ by writing that $\frac{\theta}{0.6} \geq 1$, we have that 
\begin{gather*}
    t = \frac{1.67C_1C_2\theta^*}{(\theta^*-\frac{1}{2})^2}\log_2\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right)
    \implies t = \frac{C_3\theta^*}{(\theta^*-\frac{1}{2})^2}\ln\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right),
\end{gather*}
where $C_3 = 19.35 \geq 1.67C_1C_2\log_2(e)$
satisfies the above inequality. \\\\
So now, if the condition on $t$ is satisfied, we have
\begin{gather*}
    \epsilon^2 \geq \left(\theta^*-\frac{1}{2}\right)^2 - 2\left(\theta^*-\frac{1}{2}\right)\sqrt{\frac{\log_2\left(\frac{t+1}{\delta}\right)}{2t}} \geq \left(\theta^*-\frac{1}{2}\right)^2 - 2\left(\theta^*-\frac{1}{2}\right)\frac{\left(\theta^*-\frac{1}{2}\right)}{2.2305}\\
    \implies \epsilon^2 \geq C_4\left(\theta^*-\frac{1}{2}\right)^2,
\end{gather*}
where $C_4 = 0.1033$.\\
Previously, we had remarked that it was sufficient to have
\begin{gather*}
    t \geq \frac{2\theta^*}{\epsilon^2}\ln\left(\frac{2}{\alpha}\right)
\end{gather*}
We can loosen this by using the lower bound on $\epsilon$ to: it is sufficient to satisfy
\begin{gather*}
    t \geq \frac{C_5\theta^*}{\left(\theta^*-\frac{1}{2}\right)^2}\ln\left(\frac{2}{\alpha}\right),
\end{gather*}
where $C_5 = 19.36$. \\
To make both the lower bound on $\epsilon$ and the above equation valid, we note that the following choice of $t$ works:
\begin{gather*}
    t = \frac{C_5\theta^*}{\left(\theta^*-\frac{1}{2}\right)^2}\max\left(\left(\ln\left(\frac{C_1}{(\theta^*-\frac{1}{2})^2\delta}\right), \ln\left(\frac{2}{\alpha}\right)\right)\right)
\end{gather*}
We note that, when $\alpha = \delta$, this leaves us with the following choice of $t$:

\begin{gather*}
    t = \frac{19.36\theta^*}{\left(\theta^*-\frac{1}{2}\right)^2}\left(\ln\left(\frac{2.49}{(\theta^*-\frac{1}{2})^2\delta}\right)\right)
\end{gather*}
Note that $t \geq 106$.

Combining both the above bounds, we have that
\begin{gather*}
    t = \frac{19.36\theta^*}{\left(\theta^*-\frac{1}{2}\right)^2}\left(\ln\left(\frac{2.49}{(\theta^*-\frac{1}{2})^2\delta}\right)\right)
\end{gather*}
is sufficient.\\\\
Looking over both cases, we note
\begin{gather*}
    t = \frac{20.775\theta^*}{\left(\theta^*-\frac{1}{2}\right)^2}\left(\ln\left(\frac{2.49}{(\theta^*-\frac{1}{2})^2\delta}\right)\right)
\end{gather*}
is sufficient. We denote $C_6 = 20.775, C_7 = 2.49$ to get
\begin{gather*}
    t = \frac{C_6\theta^*}{\left(\theta^*-\frac{1}{2}\right)^2}\left(\ln\left(\frac{C_7}{(\theta^*-\frac{1}{2})^2\delta}\right)\right)
\end{gather*}

==> NeurIPS submission/sections/ppr_general_proof.tex <==
\subsubsection{Generalizing Bound to $k$ Parties}
\label{sec:ppr_2}
We generalize 2-party PPR to $k$-party PPR by proposing a new algorithm named PPR-2. We first show correctness. Since we run 2-party PPR on each pair of parties, the pair $(1,j)$ giving the wrong winning party has probability at-most $\frac{\delta}{k-1}$. Using a union-bound, the probability of error is less than or equal to $\delta$. Thus, the algorithm is correct.\\\\
Consider the two party case, comparing parties $1, j$. We note that our new parameters $a, b$ will be the following:
\begin{gather*}
    a = \frac{p_1}{p_1+p_j} \\
    b = \frac{p_j}{p_1+p_j}
\end{gather*}
We consider the $(\frac{\delta}{k-1}, \frac{\alpha}{2(k-1)})$ stopping time for this pair of parties. Let us denote it as $t'$. We get
\begin{gather*}
    t' = \frac{C_6a}{\left(a-\frac{1}{2}\right)^2}\max\left(\left(\ln\left(\frac{C_7(k-1)}{(a-\frac{1}{2})^2\delta}\right), \ln\left(\frac{4(k-1)}{\alpha}\right)\right)\right)
\end{gather*}
We assume that $\alpha = \delta$. We get
\begin{gather*}
    t' = \frac{4C_6p_1(p_1+p_j)}{(p_1-p_j)^2}\left(\ln\left(\frac{C_7(k-1)}{(\frac{p_1}{p_1+p_j}-\frac{1}{2})^2\delta}\right)\right) \\
   \implies  t' \leq \frac{4C_6p_1(p_1+p_j)}{(p_1-p_j)^2}\left(\ln\left(\frac{16C_7(k-1)p_1^2}{(p_1-p_2)^2\delta}\right)\right)
\end{gather*}
We note that this two party PPR gives us a winning party with probability $1 - \frac{\alpha}{2(k-1)}$ when we reach $t'$ samples for this pair. \\\\
Let $Z_t$ be a random variable denoting how many samples are from either party $1$ or $j$. We note that $Z_t$ is a sum of $t$ bernoulli random variables with parameter $p_1+p_j$. We note that 
If we had $t$ samples in total, then we note that 
\begin{gather*}
    Pr(Z \leq (1-l)(p_1+p_j)t) \leq \exp\left(-\frac{l^2(p_1+p_j)t}{2}\right)\\
    \implies 
    Pr(Z \leq (1-l)(p_1+p_j)t) \leq \frac{\alpha}{2(k-1)}, l = \sqrt{\frac{2\ln\left(\frac{2(k-1)}{\alpha}\right)}{(p_1+p_j)t}}
\end{gather*}
Therefore, with probability $1 - \frac{\alpha}{2(k-1)}$, $Z \geq (1-l)(p_1+p_j)t$. Thus, when $t \geq \frac{t'}{(p_1+p_j)(1-l)}$, with $1 - \frac{\alpha}{2(k-1)}$ probability we have reached the $(\frac{\delta}{k-1}, \frac{\alpha}{2(k-1)})$ stopping time for the pair $(i, j)$. Using a union bound, we get that when $t \geq \frac{4C_6p_1}{(1-l)(p_1-p_2)^2}\left(\ln\left(\frac{16C_7(k-1)p_1^2}{(p_1-p_2)^2\alpha}\right)\right)$, we have $(\frac{\delta}{k-1}, \frac{\alpha}{2(k-1)})$ stopping times for all the pairs $(1, j)$, and since the total error possible is $\delta$ and we stop with probability atleast $1-\alpha$, this is an $(\delta, \alpha)$ stopping time. \\\\
We note that choosing 
\begin{gather*}
    t = \frac{C_6p_1}{(p_1-p_2)^2}\left(\ln\left(\frac{16C_7(k-1)p_1^2}{(p_1-p_2)^2\delta}\right)\right) 
    \implies
    l \leq C_7 
\end{gather*}
where $C_6 = 97.095, C_7 = 0.14357$. Thus, the following value of $t$ works:
\begin{gather*}
    t = \frac{97.03p_1}{(p_1-p_2)^2}\ln\left(\frac{39.84(k-1)p_1^2}{(p_1-p_2)^2\delta}\right) \\ 
    \implies t = \frac{194.06p_1}{(p_1-p_2)^2}\ln\left(\sqrt{\frac{39.84(k-1)}{\delta}}\frac{p_1}{(p_1-p_2)}\right) 
\end{gather*}
hence, everything is consistent and $t$ is indeed a $(\delta, \alpha)$ stopping time.\\\\
We note that this is not a bound on the expected stopping time. However, it can be converted to one by the doubling trick - we re-start the algorithm at times which are powers of $2$.

==> NeurIPS submission/sections/pprmcs.tex <==
\section{PPR Martingale Confidence Sequences}
\label{sec:pprmcs}

In this section, we consider the ``base case'' of mode estimation, in which $\mathcal{P}$ takes exactly $K = 2$ values.  Notice that $\mathcal{P}(p, v, 2)$ is a Bernoulli distribution that generates $v_{1}$ with probability $p_{1}$ and $v_{2}$ with probability $p_{2} = 1 - p_{1}$. Treating $p_{1} \in [0, 1]$ as the sole parameter of the distribution, our task is to devise a $\delta$-correct stopping rule to test if $p_{1} > \frac{1}{2}$. Since $p_{1}$ may be arbitrarily close to $\frac{1}{2}$, it is not possible to decide beforehand how many samples suffice for the test to succeed. An unfortunate consequence of having a \textit{random} stopping time is that it cannot be used directly within concentration inequalities such as Chernoff bounds. Rather, stopping rules invariably go through a union bound over all possible stopping times, dividing the mistake probability $\delta$ among them~\cite{ICML12-shivaram,pmlr-v30-Kaufmann13}. Although there has been progress towards optimising this apportioning of $\delta$~\cite{Jamieson14,garivier2013}, resulting methods still have tunable parameters in their ``decay rates'' that govern the stopping time.

The recent development of ``time-uniform'' or ``anytime'' Chernoff bounds~\cite{Howard20} relieve the experimenter of the burden of parameter-tuning. Arising from this line of research is the framework of prior-posterior-ratio (PPR) martingale confidence sequences~\cite{waudby-ramdas-ppr}, which result in a simple and intuitive stopping rule. Although the rule may be applied to a wide range of single-parameter families, we restrict our upcoming 
discussion to the Bernoulli case at hand: that is, to test whether $p_{1} > \frac{1}{2}$.

To apply the PPR martingale framework, we maintain a belief distribution $\pi$ for $p_{1}$ over its range $[0, 1]$, and update $\pi$ according to Bayes' rule as samples are observed. Our aim is still to provide a frequentist guarantee of that holds for all possible values of $p_{1}$ ($\delta$-correctness). To this end we must ensure that
the prior distribution $\pi^{0}$ gives non-zero density to all possible values of $p_{1}$. We do so by adopting the uniform prior $\pi^{0}(\hat{p}_{1}) = 1$ for $\hat{p}_{1} \in [0, 1]$. For $t \geq 1$, we update our belief distribution after observing sample $x^{t}$, as follows. 
\begin{equation*}
    \pi^{t}(\hat{p}_{1}) = \frac{\pi^{t - 1}(\hat{p}_{1}) \cdot (\hat{p}_{1})^{\mathbf{1}[x^{t} = v_{1}]} \cdot 
(1 - \hat{p}_{1})^{\mathbf{1}[x^{t} = v_{2}]}
}{\int_{\rho = 0}^{1} \pi^{t - 1}(\rho) \cdot (\rho)^{\mathbf{1}[x^{t} = v_{1}]} \cdot (1 - \rho)^{\mathbf{1}[x^{t} = v_{2}]} d\rho}.
\end{equation*}
The prior-posterior-ratio (PPR) at $\hat{p}_{1} \in [0, 1]$ is given by $R^{t}(\hat{p}_{1}) = \frac{\pi^{0}(\hat{p}_{1})}{\pi^{t}(\hat{p}_{1})}$. Making use of the fact that the PPR evaluated at the \textit{true} parameter value, $p_{1}$, is a martingale, it can be shown that the sequence of sets $(C^{t})_{t = 0}^{\infty}$, where $C^{t} \eqdef \{\hat{p}_{1}: R^{t}(\hat{p}_{1}) < \frac{1}{\delta}\}$, is a $(1 - \delta)$-confidence sequence for $p_{1}$~\cite{waudby-ramdas-ppr}. In other words, we have the ``anytime'' guarantee that 
\begin{equation}
\label{eqn:ppr-correctness}
\mathbb{P}\{\: \exists \: t \geq 0: p_{1} \notin C^{t} \} \leq \delta.
\end{equation}
The belief distribution $\pi^{t}$ and hence the PPR $R^{t}$ assume a convenient form if initialised with the uniform prior.
%\sj{The following line looks a bit awkward with the long dash}
Suppose the sequence of samples up to time $t$ is $x^{1}, x^{2}, \dots, x^{t}$, which contains $s^{t}_{1}$ occurrences of $v_{1}$ and $s^{t}_{2} = t - s_{1}$ occurrences of $v_{2}$. Then for $t \geq 0$ and $\hat{p}_{1} \in [0, 1]$, we obtain $\pi_{t}(\hat{p}_{1}) = \text{Beta}(\hat{p}_{1}; s^{t}_{1} + 1, s^{t}_{2} + 1)$. We can terminate as soon as the $(1 - \delta)$-confidence sequence on $p_{1}$ does not contain $\frac{1}{2}$. For easy readability, let us define indices $\text{first}(t)$ and $\text{second}(t)$, where $(\text{first}(t), \text{second}(t)) \in \{(1, 2), (2, 1)\}$ satisfy $s^{t}_{\text{first}(t)} \geq s^{t}_{\text{second}(t)}$. We obtain the following simple simple stopping rule, applied at each time step $t \geq 1$.
\begin{center}
\fbox{
\parbox{0.93\textwidth}{
PPR-Bernoulli: 
Stop and declare $v_{\text{first}(t)}$ as mode iff
$\text{Beta}\left(\frac{1}{2}; s^{t}_{\text{first}(t)} + 1, s^{t}_{\text{second}(t)} + 1\right) \leq \delta$.
}
}
\end{center}
The $\delta$-correctness of this stopping is immediate from \eqref{eqn:ppr-correctness}, itself a proven result~\cite{waudby-ramdas-ppr}. However, we are not aware of any existing analysis of its stopping time. We obtain the following upper bound by expanding out the Beta density function at $\frac{1}{2}$ and bounding tail probabilities using Chernoff bounds. The detailed working, which also involves steps to optimise constants, is provided in Appendix ~\ref{app:ppr-bernoulli-upperboundproof}.
\begin{lemma}[PPR-Bernoulli upper bound]
\label{lem:ppr-bernoulli-upperbound}
Fix $\delta \in (0, 1)$ and problem instance $\mathcal{P} = (p, v, 2)$. When PPR-Bernoulli is run on $\mathcal{P}$, with probability $1 - \delta$, the number of samples it observes is at most $$\frac{20.775 p_1}{(p_1-\frac{1}{2})^2}\ln\left(\frac{2.49}{(p_1-\frac{1}{2})^2 \delta}\right).$$
\end{lemma}
Like the result in Theorem~\ref{thm:a1upperbound}, the lemma upper-bounds the sample complexity only on the event that a mistake is not made. However, we can obtain an upper bound on the \textit{expected} sample complexity, with only the constants changed, by adopting a doubling trick---wherein the procedure is repeatedly performed with increasing budgets and decreasing mistake probabilities, until it terminates. The ``$p_{1}$'' in the numerator of the upper bound above can be ignored as a constant factor since $p_{1} \in (\frac{1}{2}, 1]$, but the explicit form is convenient for our generalisation to $K \geq 2$, which we take up in the next section.

It is worth noting that the LHS of the PPR-Bernoulli stopping rule can be evaluated \textit{exactly} as a rational using integer arithmetic, requiring a only lightweight incremental update after each sample. This implementation of the PPR-Bernoulli stopping rule is arguably simpler than the numerical optimisation needed by many other stopping rules, as we see shortly.

%\sj{I went through the original paper. Filtration and $N$ to me look like things defined to introduce the martingale concept and reinforce the definition of martingales/supermartingales. Unneeded here; we assume the reader knows about martingales.}

\subsection{Empirical comparison with other Stopping Rules for \texorpdfstring{$K = 2$}{}}
\label{subsec:empiricalcomparisonk2}

We present experimental results comparing PPR-Bernoulli with other stopping rules from the literature. The predominant approach is to construct lower and upper confidence bounds on $p_{1}$ that hold with probability $1 - \delta_{t}$ for each $t \geq 1$, satisfying $\sum_{t = 0}^{\infty} \delta_{t} \leq \delta$. The $\delta$-correctness of the procedure is ensured by  terminating only when the lower confidence bound exceeds $\frac{1}{2}$ or the upper confidence bound falls below $\frac{1}{2}$.  A common choice is to set $\delta_{t} = k \frac{\delta}{t^{\alpha}}$, with constants $k$ and $\alpha$ tuned for efficiency while ensuring $\delta$-correctness. As representatives of this approach, we pick the LUCB and KL-LUCB algorithms of Kaufmann and Kalyanakrishnan~\cite{pmlr-v30-Kaufmann13}. The former inverts Hoeffding's inequality to obtain lower and upper confidence bounds, while the latter uses a tighter Chernoff bound. Although these algorithms themselves are meant for bandit applications, their efficiency crucially depends on the tightness of the confidence bounds applied to each arm. The tuned confidence bounds~\cite{pmlr-v30-Kaufmann13} therefore become suitable baselines for our comparison. Details of our implementation of the LUCB and KL-LUCB confidence bounds, as well as forthcoming ones, are provided in Appendix~\ref{app:implementationdetails}. Links to code and related instructions are given in Appendix~\ref{app:code}.


With the intent of avoiding a na\"{i}ve union bound over time, Garivier applies a so-called \textit{peeling} argument to divide time into increasingly-sized slices. He obtains confidence regions by associating the random stopping time with a self-normalised process. The resulting stopping rule, which we denote KL-SN, still has a tunable parameter ``c'', which we set as recommended by Garivier~\cite{garivier2013}.

Although the $\mathcal{A}_{1}$ algorithm of Shah et al.~\cite{Shah_Choudhury_Karamchandani_Gopalan_2020} is designed specifically for mode estimation, we include it in this comparison to observe its performance when $K = 2$. In this special case, the algorithm reduces to an application of an empirical Bernstein bound given by Maurer and Pontil~\cite{maurer2009}.

%add empirical bernstein stopping
%Add bib: \url{http://icml2008.cs.helsinki.fi/papers/523.pdf} \dm{added cite as \cite{mnih2008}}.

    
In Figure~\ref{fig:bernoulli-pvaried}, we observe the stopping times of the different rules as $p_{1}$ is varied, for mistake probability $\delta = 0.01$. KL-LUCB shows a marginal improvement over (Hoeffding) LUCB, while
%the \jv{typo? change to KL-SN}
KL-SN clearly outperforms both. However, PPR-Bernoulli is significantly more efficient than even KL-SN. Given its simplicity and non-reliance on parameter-tuning, PPR-Bernoulli therefore becomes an
attractive proposition for stopping problems. Surprisingly, in spite of using variance information, $\mathcal{A}_{1}$ registers the worst performance among all the methods compared in this experiment. We attribute this result to slack in the constants used in its stopping rule, which future work can possibly tighten, while still ensuring $\delta$-correctness. Figure~\ref{fig:bernoulli-deltavaried} affirms the trend among the stopping rules when they are applied to the same distribution ($p_{1} = 0.65$), but with varying mistake probability $\delta$.\\

\begin{figure}[b]
    \centering
    \subfloat[\centering $p_1$ varied; $\delta = 0.01$. ]{{\includegraphics[width=7cm]{figures/pic1.png} }
    \label{fig:bernoulli-pvaried}}%
    % \qquad
    \subfloat[\centering $\delta$ varied; $p_{1} = 0.65$. ]{{\includegraphics[width=7cm]{figures/pic2.png} }
    \label{fig:bernoulli-deltavaried}
    }%
    \caption{Comparison of stopping rules for the Bernoulli case ($K = 2$). Both plots show sample complexity: in (a) as $p_{1}$ is varied, and in (b) as $\delta$ is varied. The results are averages from {100} runs. Error bars show one standard error (in both plots very small).
    }%
    \label{fig:fig_binary}%
\end{figure}
\vspace{-0.5cm}
    
%\jv{Updated the plots. KL-SN1 uses the exploration rate of the form $log(t^2 log(1/\delta)/\delta)$, (KL)-LUCB use a better factor for t equal to 1.1 but both the above still use union bound. KL-SN2 makes this tighter and hence lower samples. The above shall help in explaining the results  }    



% \begin{figure}[H]
%     \centering
%     \subfloat[\centering Number of samples by varying $p_1$ ]{{\includegraphics[width=7cm]{figures/updated_final_6_pvary.png} }}%
%     % \qquad
%     \subfloat[\centering Number of samples by varying $\delta$ ]{{\includegraphics[width=7cm]{figures/updated_final_6_delvary.png} }}%
%     \caption{Fig (a) compares the average number of samples needed before the stopping rule is true for a fixed error probability $\delta = 0.01$. Fig (b) studies the dependence on the $\delta$ using a fixed $p_1 = 0.65$. Note that the curves are straight lines which is justified by the log$\left(\frac{1}{\delta}\right)$ dependence and that PPR outperforms other baselines. One standard error is shown on the curves. Best viewed in color. }%
%     \label{fig:fig_binary}%
% \end{figure}


==> appendices/dirichlet.tex <==
\section{COMPARISON WITH MULTIDIMENSIONAL PPR (PPR-MD)}
\label{app:dirichlet}

The Dirichlet distribution is the conjugate prior of the Multinomial distribution, and hence can be used to implement a PPR-based stopping rule, which is similar in principle to the multi-variate PPR given in Appendix C in \cite{waudby-ramdas-ppr}. In specific, the PDF of the Dirichlet distribution is given as 
\begin{gather*}
    pdf(x) = \frac{\prod_{i=1}^{K}x_i^{\alpha_i-1}}{B(\alpha)}, \\
    B(\alpha) = \frac{\prod_i \Gamma(\alpha_i)}{\Gamma(\sum_i \alpha_i)}
\end{gather*}
At each time-step $t$, we maintain a confidence set ${C}^t$ with $x \in [0,1]^{k}$, such  that $C^{t} \eqdef \{x: R^{t}(x) < \frac{1}{\delta}\}$. We stop at time $t$ when all the $x \in C^t$ have the same unique mode. We call this stopping rule PPR-MD (Multi-dimensional). We note that, with prior $\alpha = [1, ..., 1]$,
\begin{gather*}
    R_t(x) = \frac{1}{(K-1)!}*\frac{B(\alpha)}{\prod_{i=1}^{K}x_i^{\alpha_i-1}}
\end{gather*}
We will show that if the PPR-MD stopping rule stops at a point, then PPR-1v1 would also have stopped. In other words, PPR-MD stopping \textit{implies} PPR-1v1 stopping on every run.

Let the number of observations from $v_1, v_2, ..., v_K$ until timestep $t$ be $s_1, s_2, ..., s_K$. WLOG, order them such that $s_1 \geq s_2 \geq ... \geq s_K$. We denote the empirical means as $\mu_i = \frac{s_i}{\sum_i s_i}$. We note that, when PPR-MD stops, $x_1 = (\frac{\mu_1+\mu_2}{2}, \frac{\mu_1+\mu_2}{2}, \mu_3, ..., \mu_K)$ must not lie in the confidence set. Explicitly,
\begin{gather*}
    \frac{\left(\frac{\mu_1+\mu_2}{2}\right)^{s_1+s_2}\mu_3^{s_3}...\mu_K^{s_K}}{s_1!s_2!...s_K!} \leq \frac{\delta}{(K-1)!}
\end{gather*}
We divide our proof into two parts. First, we show the implication for $K = 3$, and then we extend our proof to general $K$.


\begin{comment}
When PPR-MD stops, it must be true that,
\begin{gather*}
    max_{x \in P_{second(t)}} R_t(x) \geq \frac{1}{\delta} \\
    
\end{gather*}
where $P_{second(t)}$ is the set of distributions with $second(t)$ being the mode. We now proceed in two steps: First, we show that the Dirichlet stopping implies PPR-ME stopping when $K = 3$. Then, we show that Dirichlet stopping implies PPR-ME stopping for all $K$, by using our results from $K = 3$.
\end{comment}


\subsection{Proof for $K = 3$}
We write this down explicitly for $K = 3$. We get that, if $s_1, s_2, s_3$ are the number of observations with $s_1 \geq s_2 \geq s_3$, and $\mu_i = \frac{s_i}{\sum_i s_i}$,
\begin{gather*}
    max_{x \in P_{second(t)}} pdf(x) \leq \frac{\delta}{(K-1)!}
\end{gather*}
In particular, if we choose the point $x = \left(\frac{\mu_1+\mu_2}{2}, \frac{\mu_1+\mu_2}{2}, \mu_3\right)$, then we must have that $pdf(x) \leq \frac{\delta}{(K-1)!}$. 
PPR-ME stops when
\begin{gather*}
    \frac{\left(\frac{1}{2}\right)^{s_1+s_2}(s_1+s_2+1)!}{s_1!s_2!} \leq \frac{\delta}{2}
\end{gather*}
and Dirichlet stopping rule (using that $K = 3$) is
\begin{gather*}
    \frac{\left(\frac{\mu_1+\mu_2}{2}\right)^{s_1+s_2}\mu_3^{s_3}(s_1+s_2+s_3+2)!}{s_1!s_2!s_3!} \leq \frac{\delta}{2}
\end{gather*}
If we can show that
\begin{gather*}
    \frac{\left(\frac{\mu_1+\mu_2}{2}\right)^{s_1+s_2}\mu_3^{s_3}(s_1+s_2+s_3+2)!}{s_1!s_2!s_3!} \geq \frac{\left(\frac{1}{2}\right)^{s_1+s_2}(s_1+s_2+1)!}{s_1!s_2!},
\end{gather*}    
for all $s_1, s_2, s_3, s_1 \geq s_2 \geq s_3$, then Dirichlet stopping will imply PPR-ME stopping for $K = 3$.

 We note that this is equivalent to showing
\begin{gather*}
    \Leftrightarrow (\mu_1+\mu_2)^{s_1+s_2}\mu_3^{s_3} \geq \frac{s_3!(s_1+s_2+1)!}{(s_1+s_2+s_3+2)!} \\
    \Leftrightarrow \mu_a^{s_a}\mu_b^{s_b} \geq \frac{(s_a+1)!s_b!}{(s_a+s_b+2)!}, s_a = s_1+s_2, s_b = s_3 \\
    \Leftrightarrow \frac{s_a^{s_a}s_b^{s_b}}{(s_a+s_b)^{s_a+s_b}} \geq \frac{(s_a+1)!s_b!}{(s_a+s_b+2)!} 
\end{gather*}
for all $s_a, s_b, s_a \geq 2s_b$. \\ 

\begin{comment}
If we keep $s_b = 1$, then we have to prove
\begin{gather*}
    s_a^{s_a}*(s_a+2)(s_a+3) \geq (s_a+1)^{s_a+1} \\
    s_a + 3 \geq \left(1+\frac{1}{s_a}\right)^{s_a}
\end{gather*}
If we keep $s_b = 2$, we get
\begin{gather*}
4s_a^{s_a}*(s_a+3)(s_a+4) \geq 2*(s_a+2)^{s_a+1}
\end{gather*}
\end{comment}

Rewriting, we want to show that, when $s_b = y$, then
\begin{gather*}
    y^y(s_a+2)...(s_a+y+2) \geq y!(s_a+y)^{y}\left(1+\frac{y}{s_a}\right)^{s_a}
\end{gather*}
where $s_a \geq 2y$, $y \geq 0$. Noting that in the Dirichlet prior when $y = 0$ the $\mu_3^{s_3}$ term disappears, it is enough to show this for $y > 0$, since it is true for $y = 0$. \\
Equivalently, we want to show that 
\begin{gather*}
    f(x,y) = \frac{y^y(x+2)...(x+y+2)}{y!(x+y)^y\left(1+\frac{y}{x}\right)^x}-1 \geq 0 \text{ when } y > 0, x \geq 2y
\end{gather*}
To this end, we first show that $f(x, y)$ is an increasing function in $x$, and then we use the minimum value of $x$ for a fixed $y$ and show that at this point we satisfy that $f(x, y) \geq 0$. 

\subsubsection{Showing that $f(x, y)$ is increasing in $x$}
Recapping, we need to show that 
\begin{gather*}
    f(x,y) = \frac{y^y(x+2)...(x+y+2)}{y!(x+y)^y\left(1+\frac{y}{x}\right)^x}-1 \text{ when } y > 0, x \geq 2y
\end{gather*}
is increasing with respect to $x$ and keeping $y$ fixed. We write down the partial derivative as follows: (we remove the multiplicative positive factor purely dependent on $y$)
\begin{gather*}
    \frac{\partial f(x,y)}{\partial x} \propto \sum_{j=2}^{y}\frac{1}{x+j} - \frac{y}{x+y} + \frac{1}{x+y+2}+\frac{1}{x+y+1} + 1 - \frac{x}{x+y} - \ln\left(\frac{x+y}{x}\right) \\
    \implies \frac{\partial f(x,y)}{\partial x} \propto \sum_{j=2}^{y}\frac{1}{x+j} + \frac{1}{x+y+2}+\frac{1}{x+y+1} - \ln\left(\frac{x+y}{x}\right)
\end{gather*}
We note that
\begin{gather*}
    \frac{1}{x+j} \geq \int_{w=j}^{w=j+1}\frac{1}{x+w}dw = \ln\left(\frac{x+j+1}{x+j}\right) \\
    \sum_{j=2}^{y}\frac{1}{x+j} \geq \ln\left(\frac{x+y+1}{x+2}\right)
\end{gather*}
Thus, if we show that 
\begin{gather*}
    g(x, y) = \ln\left(\frac{x+y+1}{x+2}\right) + \frac{1}{x+y+2}+\frac{1}{x+y+1} - \ln\left(\frac{x+y}{x}\right) \geq 0 \text{ when } y > 0, x \geq 2y
\end{gather*}
this is sufficient to show that $\frac{\partial f(x, y)}{\partial x} \geq 0 \text{ when } y \geq 0, x \geq 2y$. We note that 
\begin{gather*}
    g(x, y) = \frac{1}{x+y+2}+\frac{1}{x+y+1} - \ln\left(\frac{(x+y)(x+2)}{(x+y+1)x}\right)
\end{gather*}
We will now show that keeping $x$ fixed, $g(x, y)$ is a decreasing function of $y$. Hence, it will be sufficient to consider the maximum possible value of $y$ to show that $g(x, y) \geq 0$.
% \subsubsection{Showing that $g(x,y)$ is decreasing in $y$}
We note that 
\begin{gather*}
    \frac{\partial g(x,y)}{\partial y} = -\left(\frac{3x^3+x^2(9y+11)+x(9y^2+22y+13)+3y^3+11y^2+13y+4}{(x+y)(x+y+1)^2(x+y+2)^2}\right) \\
    \implies \frac{\partial g(x,y)}{\partial y} \leq 0, y > 0, x \geq 2y \\
\end{gather*}
Hence, $g(x, y)$ is decreasing in $y$. Thus, it is enough to consider the maximal possible value of $y$ for a fixed $x$ to show that $g(x,y) \geq 0$. We note that, for a fixed $x$, the maximum possible $y$ is $\frac{x}{2}$. Hence, we have that 
\begin{gather*}
    h(x) = g(x, x/2) = \frac{2}{3x+4} + \frac{2}{3x+2} - \ln\left(\frac{3(x+2)}{(3x+2)}\right),
\end{gather*}
and we need to show that $h(x) \geq 0 \text{ when } x > 0$. We note that \begin{gather*}
    h'(x) = -\left(\frac{8(9x^2+21x+14)}{(x+2)(3x+2)^2(3x+4)^2}\right) \\
    \implies h'(x) \leq 0 \text{ when } x > 0
\end{gather*}
Thus, $h(x)$ is a decreasing function of $x$. We also note that, as $x \rightarrow \infty, h(x) \rightarrow 0$. Thus, $h(x) \geq 0 \text{ when } x > 0$. Hence, this means that $g(x, x/2) \geq 0 \implies g(x, y) \geq 0 \implies \frac{\partial f(x,y)}{\partial x} \geq 0$ which means that $f(x,y)$ is an increasing function of $x$.

\subsubsection{Showing that $f(x,y) \geq 0$}
Since $f(x,y)$ is an increasing function of $x$ when $y$ is fixed, it is sufficient to show that $f(x,y) \geq 0$ for the minimum possible value of $x$. We note that the minimum possible value of $x$ is $x = 2y$. We have
\begin{gather*}
    f(2y, y) = \frac{y^y(2y+2)...(3y+2)-y!(3y)^y\left(\frac{3}{2}\right)^{2y}}{y!(3y)^y\left(\frac{3}{2}\right)^{2y}}
\end{gather*}
The denominator is positive. We show that the numerator is positive for all $y > 0$. 
\begin{gather*}
    h(2y, y) = y^y(2y+2)...(3y+2)-y!(3y)^y\left(\frac{3}{2}\right)^{2y} \\
    h(2y, y) = y^y\left((2y+2)...(3y+2) - y!\left(\frac{27}{4}\right)^y \right)
\end{gather*}
Let 
\begin{gather*}
    c(y) = (2y+2)...(3y+2) - y!\left(\frac{27}{4}\right)^y
\end{gather*}
We will show that $c(y) > 0, y > 0$. First, We note that $c(1) > 0$. We now use induction; assume that $c(y) > 0$ for some $y$. We will show that $c(y+1) > 0$. We have that 
\begin{gather*}
    c(y) = (2y+2)...(3y+2)-y!\left(\frac{27}{4}\right)^{y} > 0 \\
    \implies d(y) = \frac{(2y+2)...(3y+2)}{y!\left(\frac{27}{4}\right)^y} > 1
\end{gather*}
We want to show that 
\begin{gather*}
    c(y+1) = (2y+4)...(3y+5) - (y+1)!\left(\frac{27}{4}\right)^{y+1} > 0 \\
    \Leftrightarrow d(y+1) = \frac{(2y+4)...(3y+5)}{(y+1)!\left(\frac{27}{4}\right)^{y+1}} > 1
\end{gather*}
We will show that 
\begin{gather*}
    e(y) = \frac{(3y+3)(3y+4)(3y+5)}{(2y+2)(2y+3)(y+1)\frac{27}{4}} > 1 \\ 
    \Leftrightarrow (3y+3)(3y+4)(3y+5) - (2y+2)(2y+3)(y+1)\frac{27}{4} > 0
\end{gather*}
We note that the last expression turns out to be a quadratic in $y$ which is always positive when $y > 0$. Hence, $e(y) > 1$ when $y > 0$. Thus, since by our induction hypothesis we have that $d(y) > 1, y > 0$ and by our proof above we have that $e(y) > 1, y > 0$, we have that $d(y)e(y) > 1, y > 0$. We note that this implies $d(y+1) = d(y)e(y) > 1$, which is what we wanted to show in our induction step. Hence, proved.
\begin{comment}
If $s_a = 2*y$, we get
\begin{gather*}
    k^k(2k+2)...(3k+2) \geq k!(3k)^k\left(\frac{3}{2}\right)^{2k}
\end{gather*}
\begin{gather*}
    (2k+2)...(3k+2) \geq k!\left(\frac{27}{4}\right)^{k}
\end{gather*}
To prove this is increasing, suppose it is true for $k$. For $k+1$, we need to show
\begin{gather*}
    (2k+4)....(3k+5) \geq (k+1)!\left(\frac{27}{4}\right)^{k+1} \\
    \frac{(3k+3)(3k+4)(3k+5)}{(2k+2)(2k+3)} \geq \frac{27}{4}(k+1)
\end{gather*}
which is true. Thus, we just need to show this is increasing in $s_a$. We have to show that
\begin{gather*}
    f(x) = \frac{k^k(x+2)...(x+k+2)} {k!(x+k)^k\left(1+\frac{k}{x}\right)^x}
\end{gather*}
\begin{gather*}
    f(x) = \frac{x^x(x+2)....(x+k+2)}{(x+k)^{x+k}}
\end{gather*}
is increasing in $x$ for all $k \geq 1, x \geq 2k$.
\begin{gather*}
    \frac{\left(\prod_{j=2}^{k}(x+j)\right)(x+k+2)(x+k+1)}{(x+k)^k}\left(\frac{x}{(x+k)}\right)^x \text{ is increasing} 
\end{gather*}

We have to show
\begin{gather*}
    \sum_{j=2}^{k}\frac{1}{x+j} - k\frac{1}{x+k} + \frac{1}{x+k+2}+\frac{1}{x+k+1} + 1 - \frac{x}{x+k} - \ln\left(\frac{x+k}{x}\right) \geq 0 \\
    \sum_{j=2}^{k}\frac{1}{x+j} + \frac{1}{x+k+2}+\frac{1}{x+k+1} - \ln\left(\frac{x+k}{x}\right) \geq 0
\end{gather*}
We know that
\begin{gather*}
    \frac{1}{x+j} \geq \int_{w=j}^{w=j+1}\frac{1}{x+w}dw = \ln\left(\frac{x+j+1}{x+j}\right) \\
    \sum_{j=2}^{k}\frac{1}{x+j} \geq \ln\left(\frac{x+k+1}{x+2}\right)
\end{gather*}
We want to show that
\begin{gather*}
    \frac{1}{x+k+2}+\frac{1}{x+k+1} - \ln\left(\frac{(x+k)(x+2)}{(x+k+1)x}\right) \geq 0, k \geq 1, x \geq 2k \\ 
    g(x, y) = \frac{1}{x+y+2}+\frac{1}{x+y+1} - \ln\left(\frac{(x+y)(x+2)}{(x+y+1)x}\right) \geq 0, y \geq 1, x \geq 2y \\
\end{gather*}
We note that 
\begin{gather*}
    \frac{\partial g(x,y)}{\partial y} = -\left(\frac{3x^3+x^2(9y+11)+x(9y^2+22y+13)+3y^3+11y^2+13y+4}{(x+y)(x+y+1)^2(x+y+2)^2}\right) \\
    \frac{\partial g(x,y)}{\partial y} \leq 0, y \geq 1, x \geq 2y \\
\end{gather*}
Thus, $g(x,y)$ is decreasing in $y$ for our range. Since we want to prove $g(x,y)\geq 0$, hence it is sufficient to consider max possible value of $y$. The max possible value of $y = \frac{x}{2}$. We have to show
\begin{gather*}
    h(x) = g(x,x/2) = \frac{2}{3x+4} + \frac{2}{3x+2} - \ln\left(\frac{3x(x+2)}{(3x+2)x}\right) \geq 0
\end{gather*}
We note that
\begin{gather*}
    h'(x) = -\left(\frac{8(9x^2+21x+14)}{(x+2)(3x+2)^2(3x+4)^2}\right)
\end{gather*}
Thus, $h(x)$ is decreasing. We note that, as $x \rightarrow \infty, h(x) \rightarrow 0$. Since $h(x)$ is decreasing, $h(2) \sim 0.0445$, and $h(\infty) = 0$ therefore $h(x) \geq 0 \: \forall \: x \geq 2$. Hence $g(x, x/2) \geq 0 \: \forall \: x \geq 2$. Hence, $g(x, y) \geq 0 \: \forall \: y \geq 1, x \geq 2y$. Hence, $f(x, k)$ is an increasing function in $x$. Hence, done.

We write this down explicitly for $K = 4$. We get that, if $s_1, s_2, s_3, s_4$ are the number of observations with $s_1 \geq s_2 \geq s_3, s_4$, and $\mu_i = \frac{s_i}{\sum_i s_i}$,
\begin{gather*}
    max_{x \in P_{second(t)}} pdf(x) \leq \frac{\delta}{(K-1)!}
\end{gather*}
where the LHS occurs at the point $x = \left(\frac{\mu_1+\mu_2}{2}, \frac{\mu_1+\mu_2}{2}, \mu_3, \mu_4\right)$. 
PPR-ME stops when
\begin{gather*}
    \frac{\left(\frac{1}{2}\right)^{s_1+s_2}(s_1+s_2+1)!}{s_1!s_2!} \leq \frac{\delta}{3}
\end{gather*}
and Dirichlet stopping rule
\begin{gather*}
    \frac{\left(\frac{\mu_1+\mu_2}{2}\right)^{s_1+s_2}\mu_3^{s_3}\mu_4^{s_4}(s_1+s_2+s_3+s_4+3)!}{s_1!s_2!s_3!s_4!} \leq \frac{\delta}{6}
\end{gather*}
We want to show that 
\begin{gather*}
    \frac{2\left(\frac{\mu_1+\mu_2}{2}\right)^{s_1+s_2}\mu_3^{s_3}\mu_4^{s_4}(s_1+s_2+s_3+s_4+3)!}{s_1!s_2!s_3!s_4!} \geq \frac{\left(\frac{\mu_1+\mu_2}{2}\right)^{s_1+s_2}\mu_3^{s_3}(s_1+s_2+s_3+2)!}{s_1!s_2!s_3!} \geq \frac{\left(\frac{1}{2}\right)^{s_1+s_2}(s_1+s_2+1)!}{s_1!s_2!} 
\end{gather*}    
Equivalent to 
\begin{gather*}
    2\mu_4^{s_4} \geq \frac{(s_1+s_2+s_3+2)!s_4!}{(s_1+s_2+s_3+s_4+3)!} \\
    2\frac{s_b^{s_b}}{(s_a+s_b)^{s_b}} \geq \frac{(s_a+2)!s_b!}{(s_a+s_b+3)!}, s_a \geq 3s_b
\end{gather*}
We already know that 
\begin{gather*}
    \frac{s_a^{s_a}s_b^{s_b}}{(s_a+s_b)^{s_a+s_b}} \geq \frac{(s_a+1)!s_b!}{(s_a+s_b+2)!}, s_a \geq 2s_b
\end{gather*}
\end{comment}
\subsection{Extending to general $K$}
For a general $K$, PPR-ME stops when 
\begin{gather*}
    \frac{\left(\frac{1}{2}\right)^{s_1+s_2}(s_1+s_2+1)!}{s_1!s_2!} \leq \frac{\delta}{K-1}
\end{gather*}
and when Dirichlet stops, it is true that (by choosing $x = \left(\frac{\mu_1+\mu_2}{2}, \frac{\mu_1+\mu_2}{2}, \mu_3, ... \mu_{K}\right)$
\begin{gather*}
    \frac{\left(\frac{\mu_1+\mu_2}{2}\right)^{s_1+s_2}\mu_3^{s_3}\mu_4^{s_4}...\mu_K^{s_K}(s_1+s_2+s_3+s_4+...+s_K+K-1)!}{s_1!s_2!s_3!s_4!...s_K!} \leq \frac{\delta}{(K-1)!}
\end{gather*}
We want to show that 
\begin{gather*}
    \frac{(K-2)!\left(\frac{\mu_1+\mu_2}{2}\right)^{s_1+s_2}\mu_3^{s_3}\mu_4^{s_4}..\mu_K^{s_K}(s_1+s_2+s_3+s_4+...+s_K+K-1)!}{s_1!s_2!s_3!s_4!...s_K!} \geq \\ \frac{\left(\frac{1}{2}\right)^{s_1+s_2}(s_1+s_2+1)!}{s_1!s_2!} 
\end{gather*}    
We will use a sequence of inequalities; we will show that
\begin{gather*}
    \frac{(K-2)!\left(\frac{\mu_1+\mu_2}{2}\right)^{s_1+s_2}\mu_3^{s_3}\mu_4^{s_4}..\mu_K^{s_K}(s_1+s_2+s_3+s_4+...+s_K+K-1)!}{s_1!s_2!s_3!s_4!...s_K!} \geq \\ \frac{(K-3)!\left(\frac{\mu_1+\mu_2}{2}\right)^{s_1+s_2}\mu_3^{s_3}...\mu_{K-1}^{s_{K-1}}(s_1+s_2+s_3+...+s_{K-1}+K-2)!}{s_1!s_2!s_3!...s_{K-1}!} \geq ... \geq \\ \frac{\left(\frac{1}{2}\right)^{s_1+s_2}(s_1+s_2+1)!}{s_1!s_2!} 
\end{gather*}   
We will show the first inequality, and the rest follow the same structure except the last (for $K = 3$), which was already shown in the subsection above. Showing the first inequality is equivalent to showing
\begin{gather*}
    (K-2)\mu_K^{s_K} \geq \frac{(s_1+s_2+...+s_{K-1}+K-2)!s_K!}{(s_1+s_2+...+s_{K}+K-1)!} \\
    \Leftrightarrow (K-2)\mu_b^{s_b} \geq \frac{(s_a+K-2)!s_b!}{(s_a+s_b+K-1)!}, s_a \geq (K-1)s_b \\
    \Leftrightarrow (K-2)\frac{s_b^{s_b}}{(s_a+s_b)^{s_b}} \geq \frac{(s_a+K-2)!s_b!}{(s_a+s_b+K-1)!}, s_a \geq (K-1)s_b
\end{gather*}
We already know that 
\begin{gather*}
    \frac{s_a^{s_a}s_b^{s_b}}{(s_a+s_b)^{s_a+s_b}} \geq \frac{(s_a+1)!s_b!}{(s_a+s_b+2)!}, s_a \geq 2s_b
\end{gather*}
In this equation, multiplying the LHS by $\frac{(K-1)(s_a+s_b)^{s_a}}{s_a^{s_a}}$ which is a factor greater than $1$, and multiplying the RHS by $\frac{(s_a+2)...(s_a+K-2)}{(s_a+s_b+3)...(s_a+s_b+K-1)}$, which is a factor lesser than $1$, we have the inequality that 
\begin{gather*}
    \frac{s_a^{s_a}}{(s_a+s_b)^{s_b}} \geq \frac{(s_a+K-2)!s_b!}{(s_a+s_b+K-1)!}, s_a \geq 2s_b
\end{gather*}
which directly implies what we wanted to show. Hence, even in the case of $K$ parties, Dirichlet stopping implies PPR-ME stopping.


\begin{comment}
\begin{gather*}
    \frac{(x+j)}{(x+k)} \text{ is increasing}, 2 \leq j \leq k \\
\end{gather*}

\begin{gather*}
    \frac{(x+k+2)(x+k+1)}{(x+k)}\left(\frac{x}{(x+k)}\right)^x \text{ is increasing} \\
    \frac{(x+j)}{(x+k)} \text{ is increasing}, 2 \leq j \leq k \\
\end{gather*}
We have to show 
\begin{gather*}
    \frac{1}{x+k+2}+\frac{1}{x+k+1}+\frac{k-1}{x+k}+\ln\left(\frac{x}{x+k}\right) \geq 0, x \geq 2k \\
    \frac{1}{x+k+2}+\frac{1}{x+k+1}+\frac{k-1}{x+k} \geq \ln\left(\frac{x+k}{x}\right), x \geq 2k
\end{gather*}
We have to show that
\begin{gather*}
    f(x,y) = \frac{1}{x+y+2}+\frac{1}{x+y+1}+\frac{y-1}{x+y}-\ln\left(\frac{x+y}{x}\right) \geq 0, x \geq 2y
\end{gather*}
We note that
\begin{gather*}
    \frac{\partial f}{\partial y} = \frac{1-y}{(x+y)^2}-\frac{1}{(x+y+1)^2}-\frac{1}{(x+y+2)^2}\\
    \implies \frac{\partial f}{\partial y} \leq 0, y \geq 1, x \geq 2y
\end{gather*}
since $f(x,y)$ is decreasing for fixed $x$ and increasing $y$, it is sufficient to prove that $f(x,y) \geq 0, y = \frac{x}{2}$, since this is the maximum value $y$ can take. We note that 
\begin{gather*}
    f(x, x/2) = \frac{2}{3x+4} + \frac{2}{3x+2} + \frac{x-2}{3x} - \ln\left(\frac{3}{2}\right)
\end{gather*}

\begin{gather*}
    f(x+1) = \frac{k^k(x+3)....(x+k+3)}{k!(x+k+1)^k\left(1+\frac{k}{x+1}\right)^{x+1}}
\end{gather*}
We want to show that
\begin{gather*}
    \frac{f(x+1)}{f(x)} \geq 1 \\
    \frac{(x+k+3)(x+k)^k\left(1+\frac{k}{x}\right)^x}{(x+2)(x+k+1)^k\left(1+\frac{k}{x+1}\right)^{x+1}} \geq 1 \\
    \frac{(x+k+3)(1-\frac{1}{x+k+1})^k\left(1+\frac{k}{x}\right)^x}{(x+2)\left(1+\frac{k}{x+1}\right)^{x+1}} \geq 1 
\end{gather*}

\begin{gather*}
    \left(1-\frac{1}{x+k+1}\right)^k \geq 1-\frac{k}{x+k+1} = \frac{x+1}{x+k+1}
\end{gather*}

It is sufficient to show that 
\begin{gather*}
    \frac{(x+k+3)(x+1)\left(1+\frac{k}{x}\right)^x}{(x+2)(x+k+1)\left(1+\frac{k}{x+1}\right)^{x+1}} \geq 1
\end{gather*}
\end{comment}

==> appendices/figures.tex <==
\newpage

\section{RATIO OF OBSERVED SAMPLE COMPLEXITY TO LOWER BOUND}
\label{app:asymptotic-plot}

In this section we plot the ratio of our experimental sample complexity (averaged over 100 iterations) and the lower bound from Theorem~\ref{thm:lowerbound}~\citep{Shah_Choudhury_Karamchandani_Gopalan_2020} for values of $\delta$ ranging from $10^{-1}$ to $10^{-201}$. The distribution we consider is $\mathcal{P}_3$ from Table \ref{tab:tab_multiK}. We observe that KLSN-1v1 appears to be asymptotically optimal, along with PPR-1v1 (which we formally proved in Appendix~\ref{app:optimality-final}) while $\mathcal{A}_{1}$-1v1 seems suboptimal. We also observe that the 1v1 variant of each algorithm performs better asymptotically than its 1vr counterpart.  


==> appendices/optimality_k_general.tex <==
\section{Proof of Optimality for General K}

Let the $D(\mathcal{P}||\mathcal{P}')$ denote the divergence term in the Sequential Mode estimation paper for a distribution with K classes. Assume the true means are $p_1 > p_2 \geq \dots p_k $ Let $D(p||0.5)$ denote the term that arises in the lower bound for K=2, with the mode having a probability p. 

\subsection{Useful Lemmas}

\subsubsection{Lemma 1}

$$(p_1+p_2)D\left(\frac{p_1}{p_1+p_2} || 0.5\right) = D(\mathcal{P}||\mathcal{P}')$$

Proof,

\begin{align*}
    (p_1+p_2)D\left(\frac{p_1}{p_1+p_2} || 0.5\right) &= p_1\log\left(\frac{p_1/(p_1+p_2)}{0.5}\right) + p_2\log\left(\frac{p_2/(p_1+p_2)}{0.5}\right) \\
    &= p_1\log\left(\frac{p_1}{(p_1+p_2)/2}\right) + p_2\log\left(\frac{p_2}{(p_1+p_2)/2}\right) \\
    &= p_1\log\left(\frac{p_1}{q}\right) + p_2\log\left(\frac{p_2}{q}\right) \\
    &= D(\mathcal{P}||\mathcal{P}')
\end{align*}

\subsubsection{Lemma 2}

Consider the following function,
$$F(p) = p_1\log\left(\frac{p_1}{(p_1+p)/2}\right) + p\log\left(\frac{p}{(p_1+p)/2}\right)$$
where $p_1$ is a constant such that $p_1 \in (0,1]$ and $p \in [0,p_1)$
\begin{align*}
    F(p) &= p_1\log(p_1) + p\log(p) - (p_1 + p)\log((p_1 + p)/2) \\
         &= p_1\log(p_1) + p\log(p) - (p_1 + p)\log(p_1 + p) + (p_1 + p)\log(2) \\
    F'(p)&= 1 + \log(p) - 1 - \log(p_1 + p) + \log(2) \\
         &= \log\left(\frac{2p}{p_1 + p}\right) < 0 \quad \forall p \in [0,p_1)
\end{align*}
\subsubsection{Lemma 3}

$$(p_1+p_i)D\left(\frac{p_1}{p_1+p_i} || 0.5\right) \geq D(\mathcal{P}||\mathcal{P}') \quad \forall p_i \in [0, p_2]$$

Proof: From Lemma 1,

\begin{align*}
(p_1+p_i)D\left(\frac{p_1}{p_1+p_i} || 0.5\right) &= p_1\log\left(\frac{p_1}{(p_1+p_i)/2}\right) + p_i\log\left(\frac{p_i}{(p_1+p_i)/2}\right) \\
&\geq p_1\log\left(\frac{p_1}{(p_1+p_2)/2}\right) + p_2\log\left(\frac{p_2}{(p_1+p_2)/2}\right) \\
&= D(\mathcal{P}||\mathcal{P}')
\end{align*}

The second line follows from Lemma 2 and from the fact that $p_2 \geq p_i$

\subsection{Actual  Proof}

For a given distribution $\mathcal{P}$, there exists $N(\mathcal{P}, \epsilon_2)$ such that 
$$E_{\alpha_1} = \left(\forall t \geq N(\mathcal{P}, \epsilon_2),\forall i \in \{1,2\dots,k\}, p_i^t - \hat{p}_i^t \leq \frac{\epsilon_2}{2} \right)$$

and $\mathbb{P}(E_{\alpha_1}) \geq 1 - \alpha_1$ \\



\noindent
Now suppose for a given $\epsilon > 0$ the number of samples completed is,

$$t^* = \frac{(1+\epsilon_1)}{D(\mathcal{P},\mathcal{P}')}\log\left(\frac{K-1}{\delta}\right) + f(\mathcal{P}, \delta, \epsilon_1, \epsilon_2)$$

\noindent
On the event $E_{\alpha_1}$ and using Lemma 2, the number of samples of arms 1 and i is

\begin{align*}
s_1^t + s_i^t &\geq (p_1 + p_i - \epsilon_2)\left(\frac{(1+\epsilon_1)}{D(\mathcal{P},\mathcal{P}')}\log\left(\frac{K-1}{\delta}\right) + f(\mathcal{P}, \delta, \epsilon_1, \epsilon_2)\right) \\
&\geq \frac{(1+\epsilon_3)}{D(p_1/(p_1+p_i),0.5)}\log\left(\frac{K-1}{\delta}\right) + f'(\mathcal{P}, \delta, \epsilon_1, \epsilon_2)
\end{align*}

\noindent
We can make the function f' large enough so that $\forall i, \mathbb{P}(\neg term_i^{t^*}) \leq \frac{\alpha_2}{K-1}$ \\


\noindent
Therefore if PPR has not terminated at time $t^*$, we must have either $\neg E_{\alpha_1}$ or $\exists i, \neg term_i^{t^*}$. Using a simple union bound the probability of either of these two events is bounded by $\alpha_1 + (K-1)*\frac{\alpha_2}{K-1} = \alpha_1 + \alpha_2$. \\

\noindent
So we finally get the condition,
$$\mathbb{P} \left(\lim_{\delta\rightarrow0}\sup\frac{\tau}{\log(1/\delta)} \leq \frac{1+\epsilon}{D\left(\mathcal{P} || \mathcal{P'}\right)} \right) \geq 1 - \alpha_1 - \alpha_2$$

==> appendices/optimalty_k2.tex <==
\section{Proof of Optimality for K = 2}

\subsection{Sufficient Condition for PPR-Bernoulli Termination}

Consider a problem instance $\mathcal{P}(p, v, 2)$ having parameters $p_1$ and $p_2 = 1 - p_1$. Let us count a sample of class $v_1$ as a "1" and that of class $v_2$ as a "0". Suppose we have made t samples in total and observed k 1s, we further define the empirical parameters $\hat{p}_1^t = \frac{k}{t}$ and $\hat{p}_2^t = \frac{t-k}{t} = 1 - \hat{p}_1^t$.

Accoriding to our stopping rule we can terminate when

\begin{align*}
\text{Beta}(0.5; k + 1, t - k + 1) &\leq \delta \\
\frac{(0.5)^k(0.5)^{t-k}(t+1)!}{(k)!(t-k)!}  &\leq \delta \\
(0.5)^k(0.5)^{t-k}(t+1)\binom{t}{k} &\leq \delta
\end{align*}

Writing the condition in this form allows us to use the following well known~\footnote{See, for example, \url{https://arxiv.org/pdf/1406.7872.pdf}.} inequality, with $\alpha = \frac{k}{t}$

\begin{equation*}
    \binom{t}{\alpha t} \leq 2^{tH_b(\alpha)}\,\, \text{where $t \in \mathbb{N}$ and $\alpha \in \left[0, \frac{1}{2}\right].$} 
\end{equation*}

The definition of binary entropy function $H_b$ for $p \in [0, 1]$ is: 
\begin{equation*}
    H_b(p) = 
    \begin{cases}
    0 & p \in \{0, 1\},\\
    -p\log_2p - (1 - p)\log_2(1 - p) & \text{otherwise.}\\
    \end{cases}
\end{equation*}

Thus we arrive at a sufficient condition for PPR-Bernoulli termination

\begin{align*}
    (0.5)^k(0.5)^{t-k}(t+1)2^{tH_b(\frac{k}{t})} &\leq \delta \\
    k\log(0.5) + (t-k)\log(0.5) + \log(t+1) + tH_b\left(\frac{k}{t}\right) &\leq \log(\delta) \\
    t\left(\frac{k}{t}\log(0.5) + \frac{(t-k)}{t}\log(0.5) - \frac{k}{t}\log\left(\frac{k}{t}\right) - \frac{(t-k)}{t}\log\left(\frac{(t-k)}{t}\right) \right) &\leq \log\left(\frac{\delta}{t+1}\right) \\
    t\left(\hat{p}_1^t\log(0.5) + (1-\hat{p}_1^t)\log(0.5) - \hat{p}_1^t\log\left(\hat{p}_1^t\right) - (1-\hat{p}_1^t)\log\left((1-\hat{p}_1^t)\right) \right) &\leq \log\left(\frac{\delta}{t+1}\right) \\
    t\left(\hat{p}\log\left(\frac{\hat{p}}{0.5}\right) + (1-\hat{p})\log\left(\frac{1-\hat{p}}{0.5}\right)\right) &\geq \log\left(\frac{t+1}{\delta}\right) \\   
    tD(\hat{p}_1^t||0.5)&\geq \log\left(\frac{t+1}{\delta}\right)
\end{align*}

\subsection{Asymptotic Bound for Samples Required under Sufficient Condition}

The arguments in this section are along the lines of those used for bandits \cite{JMLR:v17:kaufman16a}.

We fix $\epsilon$ and introduce,
$$\sigma = \max \left\{t \in \mathbb{N}^*, D\left(\hat{p}_1^t || 0.5\right) \leq  \frac{D\left(p_1 || 0.5\right)}{1 + \epsilon/2} \right\}$$


By the law of large numbers, $\mathbb{P}(\sigma < +\infty) = 1$. Hence, $\lim\limits_{n\rightarrow\infty} \mathbb{P}(\sigma \leq n) = 1$ and for every
$\alpha \in (0, 1)$ there exists $N(\epsilon, \alpha, p_1)$ such that $\mathbb{P}(\sigma \leq N(\epsilon, \alpha, p_1)) \geq 1 - \alpha$. Therefore,
introducing the event

$$E_\alpha = \left(\forall t \geq N(p, \epsilon, \alpha), D\left(\hat{p}_1^t || 0.5\right) >  \frac{D\left(p_1 || 0.5\right)}{1 + \epsilon/2}\right) \text{, one has } \mathbb{P}\left(E_\alpha\right) \geq 1 - \alpha $$

On the event $E_\alpha$,

\begin{align*}
\tau &\leq \max\left(N(\epsilon, \alpha, p_1), \inf \left\{ t \in \mathbb{N}: t\frac{D\left(p_1 || 0.5\right)}{1 + \epsilon/2} \geq \log\left(\frac{t+1}{\delta} \right)\right\}\right) \\
\tau &\leq N(\epsilon, \alpha, p_1) + \inf \left\{ t \in \mathbb{N}: t\frac{D\left(p_1 || 0.5\right)}{1 + \epsilon/2} \geq \log\left(\frac{t+1}{\delta} \right)\right\}
\end{align*}

Lemma 18 of Garivier et al. \cite{pmlr-v49-garivier16a} with $c_1 = \frac{D\left(p_1 || 0.5\right)}{1 + \epsilon/2}$, $c_2 = \frac{1}{\delta}$ and $\alpha = 1 + \gamma$ gives us the following bound

$$\tau \leq N(p, \epsilon, \alpha) + \frac{(1+\gamma)(1+\epsilon/2)}{D\left(\mathcal{P} || \mathcal{P'}\right)}\left(\log\left(\frac{e}{\delta}\left(\frac{1+\epsilon/2}{D\left(\mathcal{P} || \mathcal{P'}\right)}\right)^{1+\gamma} \right) + \log\left(\log\left(\frac{1}{\delta}\left(\frac{1+\epsilon/2}{D\left(\mathcal{P} || \mathcal{P'}\right)}\right)^{1+\gamma} \right)\right) \right)$$

We can make $\gamma$ small enough such that $(1+\gamma)(1+\epsilon/2) \leq (1 + \epsilon)$ and we have proved the condition

$$\mathbb{P} \left(\lim_{\delta\rightarrow0}\sup\frac{\tau}{\log(1/\delta)} \leq \frac{1+\epsilon}{D\left(\mathcal{P} || \mathcal{P'}\right)} \right) \geq 1 - \alpha$$

==> appendices/theorem4calculation.tex <==
\section{CALCULATION IN PROOF OF THEOREM~\ref{thm:ppr-meupperbound}} \label{app:calculationinproofoftheorempprmeupperbound}

We have to show $u < (1 - l)(p_{1} + p_{j})t$ for $t > t^{\star}$, where
\begin{align*}
u &= \frac{20.775 q_1}{(q_1-\frac{1}{2})^2}\ln\left(\frac{2.49}{(q_1-\frac{1}{2})^2 \delta^{\prime}}\right), \\
q_{1} &= \frac{p_{1}}{p_{1} + p_{j}},\\
l &= \sqrt{\frac{2 \ln(1/\delta^{\prime})}{(p_{1} + p_{j})t}}, \text{ and}\\
t^{\star} &= \frac{194.07p_1}{(p_1-p_2)^2}\ln\left(\sqrt{\frac{79.68(k-1)}{\delta}}\frac{p_1}{(p_1-p_2)}\right).
\end{align*}
First, observe that
\begin{equation*}
u = \frac{83.1p_1(p_1+p_j)}{(p_1-p_j)^2}\ln\left(\frac{9.96(p_1+p_j)^2}{(p_1-p_j)^2 \delta^{\prime}}\right) \leq \frac{83.1p_1(p_1+p_j)}{(p_1-p_2)^2}\ln\left(\frac{39.84p_1^2}{(p_1-p_2)^2 \delta^{\prime}}\right).
\end{equation*}
Thus, we have
\begin{gather*}
    \frac{u}{(p_1+p_j)t^*} < 0.85640\frac{\ln\left(\frac{39.84p_1^2}{(p_1-p_2)^2 \delta^{\prime}}\right)}{\ln\left(\frac{79.68(k-1)}{\delta}\frac{p_1^2}{(p_1-p_2)^2}\right)} = 0.85640.
\end{gather*}
It suffices to show that $l \leq 0.1436$, which is established by the steps below.
\begin{align*}
l^2 &\leq \frac{2\ln\left(1/\delta^{\prime}\right)(p_1-p_2)^2}{(p_1+p_j)97.035p_1\ln\left(\frac{79.68(k-1)p_1^2}{\delta (p_1-p_2)^2}\right)} \leq \frac{2(p_1-p_2)^2}{(p_1+p_j)97.035p_1} \leq \frac{2}{97.035} \\
&\implies l \leq \frac{1}{\sqrt{97.035/2}} < 0.1436.
\end{align*}

\newpage
\begin{comment}
\textcolor{red}{ Please see the theorem. u is defined for arms 1 and j, not 1 and 2. Rewrite these steps in terms of j instead of 2 and upper-bound the j term by the 2 term before finishing. Also, when you do u/(p1 + pj) t*, it seems like you only get half of 0.8564 as the multiplier. Did we inflate by a factor of 2, or am I missing something? }

\sj{We need to bring a sqrt inside the ln, hence you need the factor of $2$}
\sj{Proof fixed to use p1 + pj}

We show the claim for the choice
\begin{gather*}
    t^{\star} = \frac{194.07p_1}{(p_1-p_2)^2}\ln\left(\sqrt{\frac{79.68(k-1)}{\delta}}\frac{p_1}{(p_1-p_2)}\right) \\
\end{gather*}
We note that,
\begin{gather*}
    u = \frac{20.775 q_1}{(q_1-\frac{1}{2})^2}\ln\left(\frac{2.49}{(q_1-\frac{1}{2})^2 \delta^{\prime}}\right) \\
    t^{\star} = \frac{194.07p_1}{(p_1-p_2)^2}\ln\left(\sqrt{\frac{79.68(k-1)}{\delta}}\frac{p_1}{(p_1-p_2)}\right) \\
    l = \sqrt{\frac{2 \ln(1/\delta^{\prime})}{(p_{1} + p_{2})t}}
\end{gather*}
To show that 
\begin{gather*}
    u < (1 - l)(p_{1} + p_{j})t^*
\end{gather*}
We note
\begin{gather*}
    u = \frac{83.1p_1(p_1+p_2)}{(p_1-p_2)^2}\ln\left(\frac{9.96(p_1+p_2)^2}{(p_1-p_2)^2 \delta^{\prime}}\right) \leq \frac{83.1p_1(p_1+p_2)}{(p_1-p_2)^2}\ln\left(\frac{39.84p_1^2}{(p_1-p_2)^2 \delta^{\prime}}\right)
\end{gather*}
Thus, we have
\begin{gather*}
    \frac{u}{(p_1+p_2)t^*} < 0.85640\frac{\ln\left(\frac{39.84p_1^2}{(p_1-p_2)^2 \delta^{\prime}}\right)}{\ln\left(\frac{79.68(k-1)}{\delta}\frac{p_1^2}{(p_1-p_2)^2}\right)} = 0.85640
\end{gather*}
Thus, if we show that $    l \leq 0.1436$, we're done. Note that 
\begin{gather*}
    l = \sqrt{\frac{2 \ln(1/\delta^{\prime})}{(p_{1} + p_{2})t}}\\
    l^2 = \frac{2\ln\left(1/\delta^{\prime}\right)(p_1-p_2)^2}{(p_1+p_2)97.035p_1\ln\left(\frac{79.68(k-1)p_1^2}{\delta (p_1-p_2)^2}\right)} \leq \frac{2(p_1-p_2)^2}{(p_1+p_2)97.035p_1} \\ \leq \frac{2p_1^2}{p_1^2*97.035} \leq \frac{1}{\sqrt{97.035/2}} \leq 0.14357 < 0.1436
\end{gather*}
Hence, proved.


\end{comment}


==> sections/blockchains.tex <==
\section{APPLICATION: VERIFYING SMART CONTRACTS IN PERMISIONLESS BLOCKCHAINS}
\label{sec:blockhains}


\begin{figure*}[t]
    \vspace{0.3in}
    \centering
    \subfloat[\centering $K  = 2$ (single adversarial answer)]{{\includegraphics[width=6.7cm]{figures/error_bchn.png} 
    }
    \label{fig:fmax-underestimate}
    }%
    % \qquad
    \subfloat[\centering $K = 10$  ]{{\includegraphics[width=6.7cm]{figures/samples_byz_final.png}
    }
    \label{fig:adaptiveK}
    }%
    \vspace{0.3in}
    \caption{Comparisons with SPRT for the probabilistic verification of smart contracts, obtained with parameter settings
    $N = 1600$, $m = 20$, $\delta = 0.005$, $f_{max} = 0.1$. Plot (a) shows the empirical error rates of the algorithms as the true Byzantine fraction $f$ is varied, taking $K = 2$. Plot (b) shows the sample complexity of various algorithms against varying $f$, on an instance with $K = 10$ answers.}%
    \label{fig:blockchain}%
\end{figure*}

Our second application of PAC mode estimation is in a domain of growing contemporary relevance. Permissionless blockchains such as Bitcoin~\cite{NakamotoBitcoin} and Ethereum~\cite{buterin2014} %\vinay{Bitcoin does not easily allow smart contracts. Ethereum does allow them.}
allow uncertified agents to join a pool of service providers, also called \textit{nodes}.
%\vinay{In the YODA setup, there are the usual miners who normally execute all smart contracts of Ethereum. If there were no computationally intensive smart contracts then we would not need any other nodes. Ethereum does not support computationally intensive smart contracts at this time. In YODA we proposed an additional set of volunteer nodes to execute these computationally intensive smart contracts. I am not sure if we should distinguish between miners and these other volunteer nodes in this paper though.}
A recent feature that has emerged in such blockchains is the execution of ``smart contracts''~\cite{sourav2019,buterin2014}, which could include, for example, running computationally-heavy jobs such as machine learning algorithms. In an ideal world, a client who requires a computation to be performed can simply enter into a smart contract with some particular node in the blockchain, and pay a transaction cost for the service. Unfortunately, there is no guarantee that nodes in a permissionless blockchain are honest. A ``Byzantine''
%\sd{Is the term "byzantine" common in AI community? If not, we can change this to "malicious".}
(or \textit{malicious}) node could easily return a quick-to-compute, incorrect output, to the detriment of the client. 

In recent work, Das et al.~\cite{sourav2019} propose an approach for the \textit{probabilistic verification} of smart contracts. Abstractly, assume that the computation to be performed for the client is deterministic, and it has a (yet unknown) output $o_{\text{correct}}$. The proposed model accommodates any blockchain in which the fraction of Byzantine nodes is at most $f_{\max} \in [0, \frac{1}{2})$. With this assumption, it becomes feasible to give a probabilistic guarantee on obtaining the correct output. For any fixed mistake probability $\delta \in (0, 1)$, the client could ship out the computation to  $\Theta\left(\frac{1}{(\frac{1}{2} - f_{\max})^{2}}\log(\frac{1}{\delta})\right)$
%\vinay{I don't recalling having this $\Theta$ result in YODA}
nodes, and take their majority response as the answer, thereby ensuring $\delta$-correctness. Unfortunately, transaction costs can be substantial, especially those for computationally-intensive contracts. Hence, it is in the client's interest to minimise the number of nodes queried to achieve the same probabilistic guarantee. For example, a sequential procedure could potentially query fewer nodes if $f \ll f_{\max}$.

\subsection{Comparison with SPRT}
\label{subsec:comparisonwithsprt}


Our contribution in the context of this application is to propose PPR-ME as an alternative to Wald's Sequential Probability Ratio Test (SPRT)~\cite{awald1945}, which is used by Das et al.~\cite{sourav2019} for their verification procedure. This classical test finds use in many other engineering applications~\cite{kenny1991,chen2008}, some of which could also benefit from the advantages of PPR-ME over SPRT.

To apply SPRT for verifying smart contracts, Das et al.~\cite{sourav2019} assume that out of the total of $N$ nodes in the blockchain, batches of size $m$, chosen uniformly at random, can be queried in sequence.
%\sd{The term "step" is introduced suddenly. May be start with "The approach of [22] proceeds in steps, where a subset of nodes are sampled in each step"?}.
For simplicity assume the answers returned are from the set $\{0, 1, 2, \dots\}$. Let $q = \frac{m}{N}$, and $c_{i,t}$ be the number of times answer $i$ is reported in the $t^{th}$ step, $i \geq 0$, $t \geq 1$. Defining $l_{i,T} = \sum_{t=1}^{T} (2c_{i,t} - m)m$, a derivation~\cite{sourav2019} establishes that $\delta$-correct SPRT stops at time $T$, giving $i$ as the answer if
\begin{equation*}
    l_{i,T} > \ln\left ( \frac{1 - \delta}{\delta} \right) \frac{2q(1-q)N (1 - f_{\max})f_{\max}}{1 - 2f_{\max}}.
\end{equation*}
The primary disadvantage of SPRT in this context is the need for the user to provide $f_{\max}$, which is used in the stopping rule.
%\sj{Isn't the need of a large $m$ to be $\delta$-correct also a disadvantage? Whereas we give provable $\delta$-correctness with similar sample complexity}
While a lower value of $f_{\max}$ will improve the efficiency of the rule, unfortunately $\delta$-correctness no longer holds if $f$, the true fraction of Byzantine nodes, exceeds $f_{max}$. Figure~\ref{fig:fmax-underestimate} plots the empirical error made by SPRT (averaged over 50,000 runs) on a problem instance in which the Byzantine nodes all give the same (incorrect) answer. We fix $f_{\max} = 0.1$, and plot the error for different settings of $f$. The blockchain has $N = 1600$ nodes, of which SPRT samples $m = 20$ at a time. Although the test is run using  mistake probability $\delta = 0.005$, observe that the empirical error exceeds $\delta$ when $f > f_{\max}$.
%\vinay{I don't see any error bars in the Figure? Would that hurt?}

Since the verification task at hand is precisely that of PAC mode estimation, PPR-ME becomes a viable alternative, especially since it does not need the knowledge of $f_{\max}$. In fact, PPR-ME can identify the mode even if its associated probability is less than $\frac{1}{2}$ (although in this case, it can no longer be guaranteed that the mode is $o_{\text{correct}}$, since the Byzantine nodes may collude). Observe from Figure~\ref{fig:fmax-underestimate} that unlike SPRT, the empirical error rate of PPR-ME (equivalent to PPR-Bernoulli since we have set $K = 2$) remains within $\delta$ even for $f > f_{\max}$.

In Figure~\ref{fig:adaptiveK}, we compare the sample complexities of PPR-ME and SPRT. Whereas other problem parameters (including $f_{max}$) stay the same as before, we consider an instance in which $K = 10$.
%\vinay{I seem to have missed what "K" is. Haven't read the first 4 sections. I assume it is from there.}
The single correct answer is given by a $(1 - f)$-fraction of the nodes, while $9$ different incorrect answers are given by the Byzantine nodes, each equally common. The version of SPRT used is a 1vr
%\vinay{What is 1vr?}
adaptation of the basic procedure~\cite{sourav2019} to $K = 10$. First, we observe that SPRT terminates before PPR-1v1 and PPR-1vr at all values of $f$. The PPR algorithms pay this price for having to assure $\delta$-correctness at all values of $f < \frac{1}{2}$, unlike SPRT, which does so only for $f < f_{max}$. We show the performance of another PPR variant, denoted ``PPR-Adaptive'', in the same plot. In reality, we cannot be sure about the number of answers $K$ that will be returned by the blockchain's nodes--and hence cannot use it in our stopping rule. Under PPR-Adaptive, which is a 1v1 strategy, the overall mistake probability $\delta$ is divided into the \textit{infinite} sequence $k \frac{\delta}{1^{2}}, k \frac{\delta}{2^{2}}, k \frac{\delta}{3^{2}}, \dots$ (with $k = \frac{6}{\pi^{2}}$). Whenever a new answer is revealed, it is inserted into the list of possible answers, and its pairwise tests given mistake probabilities from the unused portion of the sequence. In principle, PPR-Adaptive can accommodate any number of answers, incurring only a small increase in sample complexity, as visible from Figure~\ref{fig:adaptiveK}.



%In this section, we present an application of mode estimation in a completely different domain of verifying smart contracts in permission less blockchains. The problem can be stated as follows - we want to evaluate a deterministic function $\boldsymbol{\Psi}$ and there are a total of $N$ nodes which can be queried to evaluate the function. The nodes can be divided into two types - \emph{honest} nodes which evaluate the function correctly when queried and \emph{byzantine} nodes which can be thought of as adversaries and return a wrong evaluation of the function. The goal is to correctly evaluate the function while minimizing the number of queries to be made. It is assumed that the maximum fraction of byzantine nodes $f_{max}$ is $< 1/2$ which gives us the hope to find the correct answer. The true fraction of byzantine nodes $f \leq f_{max}$ is however unknown.\newline

%We compare our approach with the SPRT stopping rule which is shown to be optimal for the above problem [CITE]. Let $m$ be the number of set of nodes queried at each time step which is known as the execution set. SPRT considers the ratio of the likelihood of two hypotheses (answer to be correct or incorrect) and stops when this exceeds $(1 - \delta)/\delta$. More formally, let $q = m/N$ and $c_{i,k}$ be the number of times answer $c_i$ was reported in the $k^{th}$ iteration. Defining $l_{i,T} = \sum_{t=1}^{T} (2c_{i,t} - m)m$, SPRT stops at time $T$ giving $c_i$ as the answer which is correct with probability at least $1 - \delta$ if
\begin{comment}
\begin{equation*}
    l_{i,T} > \text{log}\left ( \frac{1 - \delta}{\delta} \right) \frac{2q(1-q)N (1 - f_{max})f_{max}}{1 - 2f_{max}}
\end{equation*}
The issue with SPRT is that one needs to knowledge of $f_{max}$ and the correctness relies on the fact that the true fraction of the byzantine nodes $f$ is smaller than $f_{max}$. On the other hand, PPR does not need any such information and guarantees $\delta$ correctness in all regimes.
\end{comment}

%In our experiments, we set $N = 1600$ and $f_{max} = 0.1$. We assume that all the adversaries give the same incorrect evaluation of the function which would make the problem hardest. We vary $f$ from $0.05$ to $0.4$ mainly with the aim to study under specification of $f_{max}$ for the problem at hand. The above plots are averaged over $50,000$ runs. Figure~\ref{fig:blockchain}a suggests that as $f$ increases, SPRT error also increases overshooting the $\delta = 0.05$ limit while PPR is still correct for all values of $f$. Regarding the sample complexities as shown in Figure~\ref{fig:blockchain}b, we see that PPR is not that far from SPRT given that is has no additional knowledge and always outputs the correct value of the function which is important due to security reasons in the mentioned application.\newline
% \begin{figure}[H]
%     \centering
%     \includegraphics[width = 7cm]{figures/multi_answer.png}

%     \caption{$m = 20$, $\delta = 0.005$, $f_{max} = 0.1$ }%
%     \label{fig:block2}
% \end{figure}
%Next, we study the case when the byzantine nodes can give an evaluation of the function from upto $9$ incorrect answers. Thus, this can be thought of as the case of $K = 10$ using our notation. SPRT needs knowledge of this $K$ which can be handled by our framework named PPR-Adaptive. In this, on seeing the $kth$ new answer, we assign it's confidence sequence an error probability of $6\delta/(k\pi)^2$ which ensures that union bound over all $k$ is still less than $\delta$. PPR-ME and PPR-EVR are implemented assuming the knowledge of $K$ as discussed in the previous sections. 
%\jv{For multi answer case, none of the algorithms make any error so need to think whether the plot is meaningful. The adaptively allocating error budgets can be put even in the main text while describing PPR}

% \jv{The issue is correctness of SPRT assumes the execution set is large and in practice it does violate the $\delta = 0.01$ error bound. But large execution set simply means the same number of nodes samples by all algorithms in the low $f$ regime}
% Some instances where SPRT makes errors for $f> f_{max}$(averaged over 1000 runs): [see plots for $f < f_{max}$]
% \begin{enumerate}
%     \item $f_{max} = 0.1, f = 0.2, \delta = 0.01, m = 10$: SPRT accuracy 0.986000 samples 6.780000
%     \item $f_{max} = 0.1, f = 0.2, \delta = 0.01, m = 10$: PPR accuracy 1.000000 samples 9.165000
%     \item $f_{max} = 0.1, f = 0.3, \delta = 0.01, m = 20$: SPRT accuracy 0.980000 samples 12.118000
%     \item $f_{max} = 0.1, f = 0.3, \delta = 0.01, m = 20$: PPR accuracy 0.996000 samples 16.842000
    
% \end{enumerate}
% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.25]{figures/plot_1_m1.png}
%     \caption{Comparison of various algorithms for blockchain application for $\delta = 0.01$}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.25]{figures/plot_smalldelta.png}
%     \caption{Comparison of various algorithms for blockchain application for $\delta = 10^{-8}$}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \subfloat[\centering Accuracy averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_error_m.png} }}%
%     % \qquad
%     \subfloat[\centering Samples averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_samples_m.png} }}%
%     \caption{m = 2, $\delta = 0.01$, $f_{max} = 0.45$ }%
%     \label{fig:m1}%
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \subfloat[\centering Accuracy averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_error_m5.png} }}%
%     % \qquad
%     \subfloat[\centering Samples averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_samples_m5.png} }}%
%     \caption{m = 5, $\delta = 0.01$, $f_{max} = 0.45$ }%
%     \label{fig:m1}%
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \subfloat[\centering Accuracy averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_error_m5_1e-4.png} }}%
%     % \qquad
%     \subfloat[\centering Samples averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_samples_m5_1e-4.png} }}%
%     \caption{m = 5, $\delta = 10^{-4}$, $f_{max} = 0.45$ }%
%     \label{fig:m1}%
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \subfloat[\centering Accuracy averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_error_m20.png} }}%
%     % \qquad
%     \subfloat[\centering Samples averaged over 1000 runs ]{{\includegraphics[width=7cm]{figures/final_0.45_samples_m20.png} }}%
%     \caption{m = 20, $\delta = 0.01$, $f_{max} = 0.45$ }%
%     \label{fig:m1}%
% \end{figure}


==> sections/elections.tex <==
\section{APPLICATION: WINNER-FORECASTING IN INDIRECT ELECTIONS}
\label{sec:elections}

\begin{table*}[t]
\footnotesize
\centering
\scshape
  \caption{Sample complexity of various stopping rules when coupled with (1) round-robin (RR) polling of constituencies and (2) DCB. All experiments are run with mistake probability $\delta=0.01$. Values shown are averages from 10 runs, and show one standard error.  ``Seats resolved'' indicates the number of constituencies in which a winner was identified before the overall procedure terminated.}
  \label{tab:elections}  \begin{tabular}{lccccc}
    
    \toprule
    \multirow{3}{*}{Algorithm} & 
      \multicolumn{2}{c}{India-2014 (543 seats)} &
      \multicolumn{2}{c}{Bihar-2015 (242 seats)} \\
      & \multirow{2}{*}{Samples} & {Seats} & \multirow{2}{*}{Samples} & {Seats}\\
      &  & {Resolved} &  & {Resolved}\\
      \midrule
    % \multirow{2}{*}{$\mathcal{P}_1$: .5, .25 $\times$ 2} & 1vr & 1344$\pm$20 & 444$\pm$14 & 262$\pm$12\\
    %      & 1v1 & 1157$\pm$19 & 346$\pm$13 & 218$\pm$11 \\
    % \multirow{2}{*}{Uniform-PPR} & 1vr & 560815 $\pm$ 7778 & 238 $\pm$ 2 \\
    % & 1v1 & 2054171 $\pm$ 40394 & 221 $\pm$ 1\\
    RR-$\mathcal{A}_1$-1v1 & 1578946 $\pm$ 10255 & 239 $\pm$ 2 & 4201429 $\pm$ 43932  & 221 $\pm$ 1 \\
    RR-$\mathcal{A}_1$-1vr & 1767464 $\pm$ 15828 & 234 $\pm$ 1 & 4841406 $\pm$ 58188 & 222 $\pm$ 1 \\
    RR-KLSN-1v1 & 610181 $\pm$ 7072 & 240 $\pm$ 2 & 2198678 $\pm$ 44514 & 221 $\pm$ 1 \\
    RR-KLSN-1vr & 726512 $\pm$ 6186 & 236 $\pm$ 2 & 2668729 $\pm$ 47535 & 222 $\pm$ 2 \\
    RR-PPR-1v1 & \textbf{471661 $\pm$ 7373} & 241 $\pm$ 3 &\textbf{ 1813213 $\pm$ 42081 }& 221 $\pm$ 1 \\
    RR-PPR-1vr & 560815 $\pm$ 7778 & 238 $\pm$ 2 & 2054171 $\pm$ 40394 & 221 $\pm$ 1 \\\midrule
    DCB-$\mathcal{A}_1$-1v1 & 856678 $\pm$ 3935 & 182 $\pm$ 1 & 2301936 $\pm$ 36399 & 135 $\pm$ 1 \\
    DCB-$\mathcal{A}_1$-1vr & 951684 $\pm$ 5246 & 180 $\pm$ 1 & 2481552 $\pm$ 21483 & 134 $\pm$ 1 \\
    DCB-KLSN-1v1 & 325265 $\pm$ 2096 & 186 $\pm$ 2 & 1127963 $\pm$ 22191 & 139 $\pm$ 2 \\
    DCB-KLSN-1vr & 376108 $\pm$ 4067 & 181 $\pm$ 1 & 1312027 $\pm$ 22892 & 139 $\pm$ 1 \\
    DCB-PPR-1v1 & \textbf{256911 $\pm$ 2096} & 188 $\pm$ 1 & \textbf{883389 $\pm$ 15581} & 142 $\pm$ 2 \\
    DCB-PPR-1vr & 296580 $\pm$ 2372 & 184 $\pm$ 1 & 993495 $\pm$ 18859 & 139 $\pm$ 1 \\
    \bottomrule
  \end{tabular}
%  \vspace{0.1cm}
\normalsize
\end{table*}
Opinion polls---deployed  to gauge public perception of competing products in a market, or to forecast the winner of an upcoming election---are a natural application of mode estimation. In fact, the algorithms discussed in Section~\ref{sec:ppr-me} can all be applied with only minor alterations to  \textit{plurality} systems, wherein the task is precisely that of determining the choice preferred by the largest fraction of the target population. Waudby-Smith and Ramdas~\cite{waudby-ramdas-ppr} illustrate the use of PPR martingale confidence sequences precisely on this application. Specifically they consider the construction of confidence sequences when polls receive \textit{without-replacement} samples from finite populations.

In parliamentary democracies such as India~\cite{rajeeva2002} and the United Kingdom~\cite{payne2003}, individuals in each \textit{constituency} (or \textit{seat})---typically a geographically contiguous region---elect a party based on plurality; the party winning the most seats forms the government. This two-level structure is followed both to elect governments in each state, and for the entire country. Forecasting the winning party in such an \textit{indirect} voting system calls for a more sophisticated sampling procedure. Whereas it would \textit{suffice} to separately identify the winner from each seat by sampling, it might be wasteful to do so when the overall winning party has a clear majority in its number of seats. Rather, one could potentially use the results currently available from \textit{all} the constituencies to decide which ones to query next. 

In this section, we consider a procedure that 
(1) keeps track of the current winners and leaders at the aggregate level, and (2) at each step samples the constituencies that appear most promising to confirm the aggregate trend. In principle, this algorithm, denoted DCB (for ``Difference in Confidence Bounds'') can be coupled with any algorithm that uses confidence bounds for mode estimation. Yet, we obtain the best results when DCB uses PPR-ME as a subroutine, thereby highlighting the relevance of PPR-ME not only as a stopping rule, but also as an input to on-line decision making.

DCB takes cue from the LUCB algorithm for best-arm identification in bandits~\cite{ICML12-shivaram}. At each step $t$, it identifies two parties, $a^{t}$ and $b^{t}$, that appear the most promising to win the overall election: these parties are picked based on their current number of wins and ``leads'' in individual constituencies. Subsequently the algorithm chooses a constituency each for $a^{t}$ and $b^{t}$, samples from which could ``most'' help distinguish the tally of the two. We provide a detailed specification of DCB in Appendix~\ref{app:dcbalgorithm}.

%In this section, we consider the setting of two level elections. In such an election we have several political parties contesting for a national level post such as that of the President or Prime Minister. However individuals vote to elect candidates (from different parties) to represent only their own constituency. The candidate with the most votes is elected at the constituency level, thus here we are left with the task of mode estimation. Our goal however is to predict the winner of the overall election, i.e. the party that wins the most constituencies. 

%In achieving this goal we seek to minimize the number of samples, that is, the number of voters polled. We propose an algorithm called DCB (Difference in Confidence Bounds which tells us which constituency to sample from. We show that it comprehensively outperforms a round robin baseline, i.e., sampling votes from each constituency evenly. The details of the algorithm are given below - 

\vspace{-0.2cm}

\subsection{Performance when Coupled with DCB}
\label{subsec:evaluation}

We compare DCB with a round-robin strategy for picking the next constituency to sample. Both approaches can be implemented with different stopping rules, which are also varied. Table~\ref{tab:elections} shows our results on two recent (and contrasting) elections conducted in India.\footnote{Election results are in the public domain; the authors accessed them at \url{https://www.indiavotes.com/}.} In the 2014 national elections, the winning party secured 282 seats from among 543, giving it a very large victory over the second-place party, which won 44 seats. The second problem instance is from a closer contest in the state of Bihar, in which the top three parties won 80, 71, and 53 seats, of a total 242.

While it is not the central feature of this paper, it is worth noting that the DCB strategy indeed improves over round-robin polling by roughly a factor of two, regardless of the stopping rule. As intended, it does not waste samples on constituencies that are inconsequential to the overall result (observed in the ``seats resolved'' columns). Of more direct relevance to the theme of the paper is that even when embedded within a decision-making outer loop, PPR continues to outperform $\mathcal{A}_{1}$ and KL-SN, and the 1v1 approach still dominates 1vr.

It must be emphasised that in practice, election surveys typically have the financial budget only for a few thousands of samples, and the time only for a single-stage (non-sequential) poll~\cite{karandikar2018}. Opinion polls must also cope with difficulties in obtaining truthful votes and samples drawn uniformly at random from a population~\cite{paul1979}. We have conveniently assumed a more abstract setting primarily to tease apart the efficiency of different stopping rules for mode estimation. We believe the numerical superiority of PPR-1v1 makes it a good choice for embedding within more complex and realistic models, although we leave the exercise of doing so to future work.

\begin{comment}
\begin{table}[H]
\centering
\scshape
  \begin{tabular}{lccccc}
    
    \toprule
    \multirow{3}{*}{Algorithm} & 
      \multicolumn{2}{c}{India-2014} &
      \multicolumn{2}{c}{Bihar-2015} \\
      & \multirow{2}{*}{Samples} & {Seats} & \multirow{2}{*}{Samples} & {Seats}\\
      &  & {Resolved} &  & {Resolved}\\
      \midrule
    % \multirow{2}{*}{$\mathcal{P}_1$: .5, .25 $\times$ 2} & 1vr & 1344$\pm$20 & 444$\pm$14 & 262$\pm$12\\
    %      & 1v1 & 1157$\pm$19 & 346$\pm$13 & 218$\pm$11 \\
    % \multirow{2}{*}{Uniform-PPR} & 1vr & 560815 $\pm$ 7778 & 238 $\pm$ 2 \\
    % & 1v1 & 2054171 $\pm$ 40394 & 221 $\pm$ 1\\
    Uniform-PPR & 560815 $\pm$ 7778 & 238 $\pm$ 2 & 2054171 $\pm$ 40394 & 221 $\pm$ 1 \\
    Uniform-PPR-ME & 471661 $\pm$ 7373 & 241 $\pm$ 3 & 1813213 $\pm$ 42081 & 221 $\pm$ 1 \\
    Uniform-$\mathcal{A}_1$ & 1767464 $\pm$ 15828 & 234 $\pm$ 1 & 4841406 $\pm$ 58188 & 222 $\pm$ 1 \\
    Uniform-$\mathcal{A}_1$-EVE & 1578946 $\pm$ 10255 & 239 $\pm$ 2 & 4201429 $\pm$ 43932  & 221 $\pm$ 1 \\
    Uniform-KLSN & 726512 $\pm$ 6186 & 236 $\pm$ 2 & 2668729 $\pm$ 47535 & 222 $\pm$ 2 \\
    Uniform-KLSN-EVE & 610181 $\pm$ 7072 & 240 $\pm$ 2 & 2198678 $\pm$ 44514 & 221 $\pm$ 1 \\ \midrule
    DCB-PPR & 296580 $\pm$ 2372 & 184 $\pm$ 1 & 993495 $\pm$ 18859 & 139 $\pm$ 1 \\
    DCB-PPR-ME & 256911 $\pm$ 2096 & 188 $\pm$ 1 & 883389 $\pm$ 15581 & 142 $\pm$ 2 \\
    DCB-$\mathcal{A}_1$ & 951684 $\pm$ 5246 & 180 $\pm$ 1 & 2481552 $\pm$ 21483 & 134 $\pm$ 1 \\
    DCB-$\mathcal{A}_1$-EVE & 856678 $\pm$ 3935 & 182 $\pm$ 1 & 2301936 $\pm$ 36399 & 135 $\pm$ 1 \\
    DCB-KLSN & 376108 $\pm$ 4067 & 181 $\pm$ 1 & 1312027 $\pm$ 22892 & 139 $\pm$ 1 \\
    DCB-KLSN-EVE & 325265 $\pm$ 2096 & 186 $\pm$ 2 & 1127963 $\pm$ 22191 & 139 $\pm$ 2 \\
    \bottomrule
  \end{tabular}
  \caption{Performance of various algorithms in terms of its sample complexity for determining the winner of election when $\delta=0.01$. Seats resolved indicates the number of constituencies in which winner was declared}
\end{table}
\end{comment}

==> sections/elections_new.tex <==
\section{APPLICATION: WINNER-FORECASTING IN INDIRECT ELECTIONS}
\label{sec:elections}

\begin{table}[t]
\footnotesize
\centering
\scshape
  \caption{Sample complexity of various stopping rules when coupled with (1) round-robin (RR) polling of constituencies and (2) DCB. All experiments are run with mistake probability $\delta=0.01$. Values shown are averages from 10 runs, and show one standard error.  ``Seats resolved'' indicates the number of constituencies in which a winner was identified before the overall procedure terminated.}
  \label{tab:elections-india}  \begin{tabular}{lccccc}
    
    \toprule
    \multirow{3}{*}{Algorithm} & 
      \multicolumn{2}{c}{India-2014 (543 seats)} &
      \\
      & \multirow{2}{*}{Samples} & {Seats}\\
      &  & {Resolved} \\
      \midrule
    % \multirow{2}{*}{$\mathcal{P}_1$: .5, .25 $\times$ 2} & 1vr & 1344$\pm$20 & 444$\pm$14 & 262$\pm$12\\
    %      & 1v1 & 1157$\pm$19 & 346$\pm$13 & 218$\pm$11 \\
    % \multirow{2}{*}{Uniform-PPR} & 1vr & 560815 $\pm$ 7778 & 238 $\pm$ 2 \\
    % & 1v1 & 2054171 $\pm$ 40394 & 221 $\pm$ 1\\
    RR-$\mathcal{A}_1$-1v1 & 1578946 $\pm$ 10255 & 239 $\pm$ 2 \\
    RR-$\mathcal{A}_1$-1vr & 1767464 $\pm$ 15828 & 234 $\pm$ 1 \\
    RR-KLSN-1v1 & 610181 $\pm$ 7072 & 240 $\pm$ 2 \\
    RR-KLSN-1vr & 726512 $\pm$ 6186 & 236 $\pm$ 2 \\
    RR-PPR-1v1 & \textbf{471661 $\pm$ 7373} & 241 $\pm$ 3 \\
    RR-PPR-1vr & 560815 $\pm$ 7778 & 238 $\pm$ 2  \\\midrule
    DCB-$\mathcal{A}_1$-1v1 & 856678 $\pm$ 3935 & 182 $\pm$ 1 \\
    DCB-$\mathcal{A}_1$-1vr & 951684 $\pm$ 5246 & 180 $\pm$ 1 \\
    DCB-KLSN-1v1 & 325265 $\pm$ 2096 & 186 $\pm$ 2 \\
    DCB-KLSN-1vr & 376108 $\pm$ 4067 & 181 $\pm$ 1 \\
    DCB-PPR-1v1 & \textbf{256911 $\pm$ 2096} & 188 $\pm$ 1 \\
    DCB-PPR-1vr & 296580 $\pm$ 2372 & 184 $\pm$ 1 \\
    \bottomrule
  \end{tabular}
%  \vspace{0.1cm}
\normalsize
\end{table}


Opinion polls---deployed  to gauge public perception of competing products in a market, or to forecast the winner of an upcoming election---are a natural application of mode estimation. In fact, the algorithms discussed in Section~\ref{sec:ppr-me} can all be applied with only minor alterations to  \textit{plurality} systems, wherein the task is precisely that of determining the choice preferred by the largest fraction of the target population. Waudby-Smith and Ramdas~\cite{waudby-ramdas-ppr} illustrate the use of PPR martingale confidence sequences precisely on this application. Specifically they consider the construction of confidence sequences when polls receive \textit{without-replacement} samples from finite populations.

In parliamentary democracies such as India~\cite{rajeeva2002} and the United Kingdom~\cite{payne2003}, individuals in each \textit{constituency} (or \textit{seat})---typically a geographically contiguous region---elect a party based on plurality; the party winning the most seats forms the government. This two-level structure is followed both to elect governments in each state, and for the entire country. Forecasting the winning party in such an \textit{indirect} voting system calls for a more sophisticated sampling procedure. Whereas it would \textit{suffice} to separately identify the winner from each seat by sampling, it might be wasteful to do so when the overall winning party has a clear majority in its number of seats. Rather, one could potentially use the results currently available from \textit{all} the constituencies to decide which ones to query next. 

In this section, we consider a procedure that 
(1) keeps track of the current winners and leaders at the aggregate level, and (2) at each step samples the constituencies that appear most promising to confirm the aggregate trend. In principle, this algorithm, denoted DCB (for ``Difference in Confidence Bounds'') can be coupled with any algorithm that uses confidence bounds for mode estimation. Yet, we obtain the best results when DCB uses PPR-ME as a subroutine, thereby highlighting the relevance of PPR-ME not only as a stopping rule, but also as an input to on-line decision making.

DCB takes cue from the LUCB algorithm for best-arm identification in bandits~\cite{ICML12-shivaram}. At each step $t$, it identifies two parties, $a^{t}$ and $b^{t}$, that appear the most promising to win the overall election: these parties are picked based on their current number of wins and ``leads'' in individual constituencies. Subsequently the algorithm chooses a constituency each for $a^{t}$ and $b^{t}$, samples from which could ``most'' help distinguish the tally of the two. We provide a detailed specification of DCB in Appendix~\ref{app:dcbalgorithm}.

%In this section, we consider the setting of two level elections. In such an election we have several political parties contesting for a national level post such as that of the President or Prime Minister. However individuals vote to elect candidates (from different parties) to represent only their own constituency. The candidate with the most votes is elected at the constituency level, thus here we are left with the task of mode estimation. Our goal however is to predict the winner of the overall election, i.e. the party that wins the most constituencies. 

%In achieving this goal we seek to minimize the number of samples, that is, the number of voters polled. We propose an algorithm called DCB (Difference in Confidence Bounds which tells us which constituency to sample from. We show that it comprehensively outperforms a round robin baseline, i.e., sampling votes from each constituency evenly. The details of the algorithm are given below - 

\vspace{-0.2cm}

\subsection{Performance when Coupled with DCB}
\label{subsec:evaluation}

We compare DCB with a round-robin strategy for picking the next constituency to sample. Both approaches can be implemented with different stopping rules, which are also varied. Table~\ref{tab:elections} shows our results on two recent (and contrasting) elections conducted in India.\footnote{Election results are in the public domain; the authors accessed them at \url{https://www.indiavotes.com/}.} In the 2014 national elections, the winning party secured 282 seats from among 543, giving it a very large victory over the second-place party, which won 44 seats. The second problem instance is from a closer contest in the state of Bihar, in which the top three parties won 80, 71, and 53 seats, of a total 242.

While it is not the central feature of this paper, it is worth noting that the DCB strategy indeed improves over round-robin polling by roughly a factor of two, regardless of the stopping rule. As intended, it does not waste samples on constituencies that are inconsequential to the overall result (observed in the ``seats resolved'' columns). Of more direct relevance to the theme of the paper is that even when embedded within a decision-making outer loop, PPR continues to outperform $\mathcal{A}_{1}$ and KL-SN, and the 1v1 approach still dominates 1vr.

It must be emphasised that in practice, election surveys typically have the financial budget only for a few thousands of samples, and the time only for a single-stage (non-sequential) poll~\cite{karandikar2018}. Opinion polls must also cope with difficulties in obtaining truthful votes and samples drawn uniformly at random from a population~\cite{paul1979}. We have conveniently assumed a more abstract setting primarily to tease apart the efficiency of different stopping rules for mode estimation. We believe the numerical superiority of PPR-1v1 makes it a good choice for embedding within more complex and realistic models, although we leave the exercise of doing so to future work.

\begin{comment}
\begin{table}[H]
\centering
\scshape
  \begin{tabular}{lccccc}
    
    \toprule
    \multirow{3}{*}{Algorithm} & 
      \multicolumn{2}{c}{India-2014} &
      \multicolumn{2}{c}{Bihar-2015} \\
      & \multirow{2}{*}{Samples} & {Seats} & \multirow{2}{*}{Samples} & {Seats}\\
      &  & {Resolved} &  & {Resolved}\\
      \midrule
    % \multirow{2}{*}{$\mathcal{P}_1$: .5, .25 $\times$ 2} & 1vr & 1344$\pm$20 & 444$\pm$14 & 262$\pm$12\\
    %      & 1v1 & 1157$\pm$19 & 346$\pm$13 & 218$\pm$11 \\
    % \multirow{2}{*}{Uniform-PPR} & 1vr & 560815 $\pm$ 7778 & 238 $\pm$ 2 \\
    % & 1v1 & 2054171 $\pm$ 40394 & 221 $\pm$ 1\\
    Uniform-PPR & 560815 $\pm$ 7778 & 238 $\pm$ 2 & 2054171 $\pm$ 40394 & 221 $\pm$ 1 \\
    Uniform-PPR-ME & 471661 $\pm$ 7373 & 241 $\pm$ 3 & 1813213 $\pm$ 42081 & 221 $\pm$ 1 \\
    Uniform-$\mathcal{A}_1$ & 1767464 $\pm$ 15828 & 234 $\pm$ 1 & 4841406 $\pm$ 58188 & 222 $\pm$ 1 \\
    Uniform-$\mathcal{A}_1$-EVE & 1578946 $\pm$ 10255 & 239 $\pm$ 2 & 4201429 $\pm$ 43932  & 221 $\pm$ 1 \\
    Uniform-KLSN & 726512 $\pm$ 6186 & 236 $\pm$ 2 & 2668729 $\pm$ 47535 & 222 $\pm$ 2 \\
    Uniform-KLSN-EVE & 610181 $\pm$ 7072 & 240 $\pm$ 2 & 2198678 $\pm$ 44514 & 221 $\pm$ 1 \\ \midrule
    DCB-PPR & 296580 $\pm$ 2372 & 184 $\pm$ 1 & 993495 $\pm$ 18859 & 139 $\pm$ 1 \\
    DCB-PPR-ME & 256911 $\pm$ 2096 & 188 $\pm$ 1 & 883389 $\pm$ 15581 & 142 $\pm$ 2 \\
    DCB-$\mathcal{A}_1$ & 951684 $\pm$ 5246 & 180 $\pm$ 1 & 2481552 $\pm$ 21483 & 134 $\pm$ 1 \\
    DCB-$\mathcal{A}_1$-EVE & 856678 $\pm$ 3935 & 182 $\pm$ 1 & 2301936 $\pm$ 36399 & 135 $\pm$ 1 \\
    DCB-KLSN & 376108 $\pm$ 4067 & 181 $\pm$ 1 & 1312027 $\pm$ 22892 & 139 $\pm$ 1 \\
    DCB-KLSN-EVE & 325265 $\pm$ 2096 & 186 $\pm$ 2 & 1127963 $\pm$ 22191 & 139 $\pm$ 2 \\
    \bottomrule
  \end{tabular}
  \caption{Performance of various algorithms in terms of its sample complexity for determining the winner of election when $\delta=0.01$. Seats resolved indicates the number of constituencies in which winner was declared}
\end{table}
\end{comment}
